Reverse Diffusion Monte Carlo

We propose a Monte Carlo sampler from the reverse diffusion process. Unlike the practice of diffusion models, where the intermediary updates -- the score functions -- are learned with a neural network, we transform the score matching problem into a mean estimation one. By estimating the means of the regularized posterior distributions, we derive a novel Monte Carlo sampling algorithm called reverse diffusion Monte Carlo (rdMC), which is distinct from the Markov chain Monte Carlo (MCMC) methods. We determine the sample size from the error tolerance and the properties of the posterior distribution to yield an algorithm that can approximately sample the target distribution with any desired accuracy. Additionally, we demonstrate and prove under suitable conditions that sampling with rdMC can be significantly faster than that with MCMC. For multi-modal target distributions such as those in Gaussian mixture models, rdMC greatly improves over the Langevin-style MCMC sampling methods both theoretically and in practice. The proposed rdMC method offers a new perspective and solution beyond classical MCMC algorithms for the challenging complex distributions.

==> 0_contents/020relatedwork_backup.tex <==
\section{Preliminaries}

In this section, we begin by introducing related work from the perspectives of Markov Chain Monte Carlo (MCMC) and diffusion models, and we discuss the connection between these works and the present paper. We then provide a notation formulation for the reverse process of diffusion models, which presents the stochastic differential equation (SDE) that particles follow in \textsc{rdMC}.

\subsection{Related Works}
\label{sec:related_work}
%\textcolor{blue}{Shorten this part. Combine all the MCMC samplers into one paragraph.}

%The investigation un algorithms has been a longstanding concern within the sampling community. The analysis primarily revolves around quantifying the gradient complexity or iteration complexity when the underlying distribution of output particles closely approximates the target distribution $p_\propto \exp(-f_*)$, as determined by specific criteria such as total variation, Wasserstein distances, and KL divergence. We briefly summarize the previous work to demonstrate our novelty.
%In the following paragraphs, we introduce the related work for different algorithms when the target distribution $p_*$ satisfies various assumptions.

\paragraph{Langevin-based MCMC.} The mainstream gradient-based sampling algorithms mainly follows from the continuous Langevin dynamics, i.e., 
\begin{equation*}
    \der \rvx_t = -\grad f_*(\rvx_t)\der t + \sqrt{2}\der B_t.
\end{equation*}
when it is required to sample from the target distribution $p_*\propto \exp(-f_*)$.
The Unadjusted Langevin Algorithm (ULA) utilizes the Euler-Maruyama scheme to discretize the above SDE and obtain a biased stationary distribution.
While due to its concise form and good properties, ULA is widely used in machine learning, and the convergence is investigated for different criteria, including Total Variation (TV) distance, Wasserstein distances \citep{durmus2019high}, and Kullback–Leible (KL) divergence \citep{dalalyan2017further, cheng2018convergence,ma2019sampling,freund2021convergence}.

\textcolor{blue}{\hrule}

Langevin Algorithms is the most widely use Markov chain Monte Carlo (MCMC) sampling algorithms, which generate samples with gradient-based methods in probabilistic space. The main techniques include the Langevin dynamics and the gradient flow in Wasserstein space.
The Unadjusted Langevin Algorithm (ULA) is a popular inexact discretization of the Langevin dynamics, which is widely used in machine learning. The convergence of ULA has been proved wrt total variation, Wasserstein distances \citep{durmus2019high}, and KL divergence \citep{dalalyan2017further, cheng2018convergence,ma2019sampling,freund2021convergence}.
%While ULA is known to converge to a biased limit with respect to the target distribution $p_*$, the nature and extent of this bias have been the subject of much research in recent years.
%When $p_*$ is strongly log-concave and smooth, it is possible to control the bias of ULA and prove convergence in different distance metrics, including total variation, Wasserstein distances  \citep{durmus2019high}, and KL divergence \citep{dalalyan2017further, cheng2018convergence}.Moreover, recent work has extended ULA to stochastic or inexact variants, leading to sharper results \citep{dalalyan2019user,durmus2019analysis}.Beyond the strong log-concavity,~\citet{vempala2019rapid,chewi2021analysis} provide the convergence of R\'enyi divergence when $p_*$ satisfies smoothness and isoperimetry, namelyeither the log-Sobolev or Poincar\'e inequality. Recently, with only Lipschitz gradient, %\citet{balasubramanian2022towards}showed the convergence of Fisher information along ULA, \citet{balasubramanian2022towards} undertook an analysis of the convergence properties of ULA within the framework of Fisher divergence, which is an analog of finding a first-order stationary point in non-convex optimization. However, a significant knowledge gap still remains regarding the establishment of a connection between Fisher divergence and common statistical distances in the absence of isoperimetric inequalities.Another popular technical route is Underdamped Langevin Dynamics (ULD) which is an inexact discretization of second-order SDE.\cite{cheng2018underdamped} improves the computational complexity of Wasserstein 2 convergence along ULD w.r.t. accuracy, dimension of variables, and the condition number of the negative logarithm of the target distribution, i.e., $f$. Similar rapid Wasserstein 2 convergences are provided by ULD~\citep{dalalyan2020sampling, mou2021high}, MALA~\citep{dwivedi2018log}, HMC~\citep{lee2018algorithmic, chen2022optimal} based methods.Moreover,~\citet{cao2020complexity} showed that the information complexity lower bound of randomized ULD has been achieved by~\citet{shen2019randomized}.Besides, the KL convergence of ULD is also explored by~\citet{ma2021there, zhang2023improved} when the target distribution $p_*$ satisfies smoothness and isoperimetry. To the best of our knowledge, neither ULA nor ULD can  guarantee the convergence of statistical distances mentioned before without isoperimetry. 
%\citet{balasubramanian2022theory} undertook an analysis of the convergence properties of the Langevin algorithm within the framework of Fisher divergence. However, a significant knowledge gap still remains regarding the establishment of a connection between Fisher divergence and common statistical distances in the absence of isoperimetric inequalities.
%\noindent\textbf{Proximal Samplers.}
Recently, several samplers requiring proximal oracles have been proposed to achieve better complexity.
~\citet{wibisono2019proximal} achieves the rapid convergence when the optimum of proximal subproblem w.r.t $f$ is given.
\citet{lee2021structured,chen2022improved} provide a linear convergence of Wasserstein-2 distance and KL divergence via proximal reduction framework (requiring Restricted Gaussian Oracle).
Although proximal samplers seem to have a good property in convergence, proximal oracles are usually unknown in real practice. 
To solve this problem, \citet{liang2022proximal} replaced the proximal oracles with implementable proximal bundle methods, while only the total variation distance to the target density can be guaranteed with a polynomial-time complexity.
Besides,~\citep{chen2022improved,altschuler2023faster} extends proximal samplers to cases that target distributions satisfy isoperimetry.
We emphasize the crucial observation that the proximal sampler bears a fundamental equivalence to the posterior distribution $q(\rvx_0|\rvx)$. It is noteworthy that an intriguing avenue for future research is the exploration of the intricate relationship between diffusion models and the proximal sampler. This connection represents an open question that holds immense potential for shedding light on the underlying mechanisms and theoretical foundations that unite these two concepts. 
%It is important to point out that the proximal sampler is equivalent to the posterior $q(\rvx_0|\rvx)$ in our paper. It remains open to further draw the connection between the diffusion models and the proximal sampler.
When the true distribution $p_*$ exhibits strong log-concavity, it is noteworthy that there exist alternative sampling algorithms, distinct from previous methods, that offer provable rapid convergence in terms of Wasserstein distance. Notably, these algorithms encompass the ball walk and hit-and-run techniques, as expounded upon by \cite{kannan1997random, lovasz2006fast, lovasz2007geometry, lovasz2004hit}.
\citet{holzmuller2023convergence} contributed to the field by providing a comprehensive analysis of certain samplers without relying on isoperimetry. However, it is important to acknowledge that their analysis primarily focuses on compact domains and is susceptible to the curse of dimensionality, limiting its applicability in high-dimensional settings. \citet{liu2016stein,dong2023particlebased} also attempt to perform sampling tasks with deterministic algorithm, but the limiting ODE is still derived from the Langevin dynamics. 
Unlike MCMC, our algorithm is not based time-homogeneous Markov operator, so that we can design our algorithm across time steps. Specifically, our proposed reversed SDE is more adapted to multi-modal distributions and distribution with small log-Sobolev constants.
\xunp{should we demonstrate the connection between MCMC and our method? I think only introduce MCMC is not enough. maybe from the convergence condition and properties perspective?}

\noindent\textbf{Score-based Generative Models and Stochastic Localization.}
Recent years have seen a surge in the popularity of score-based generative models and diffusion models \citep{ho2020denoising,song2020score} as they can generate high-quality real samples. Unlike traditional sampling tasks, which involve computing the density of an unnormalized distribution, the aim of generative modeling is to sample from an unknown data distribution using some real samples. 
The inference process of diffusion models~\citep{ho2020denoising} is a sampling process induced by the reverse SDE of the OU process.
Notably, the convergence properties of this inference process have been rigorously established in recent studies such as \citep{chen2022sampling,chen2022improved,lee2022convergence,lee2023convergence}, provided that accurate approximations of the score function are attainable.
It is paramount to acknowledge that diffusion models possess the remarkable ability to generate high-quality samples, even for data distributions characterized by significant irregularities. This capability stems from the distinctive nature of the reverse SDE employed in diffusion models, which sets it apart from conventional MCMC trajectories. This unique characteristic empowers the reverse SDE to excel at sampling tasks, particularly when confronted with challenging distributions.
Given these compelling characteristics, we propose harnessing the power of the diffusion process, specifically the reverse SDE associated with the inference process in diffusion models, to perform unnormalized sampling for intricate target distributions. Our motivation is to leverage this potent sampling technique to address real-world problems and showcase its superior performance in comparison to traditional methods. On the other hand, stochastic localization framework \citep{eldan2013thin,eldan2020taming,eldan2022analysis,el2022sampling,montanari2023sampling} also formalize the general reverse diffusion and discuss the relationship with current diffusion models. \citet{montanari2023posterior} consider the posterior sampling for symmetric spiked model. However, for the properties of the general unnormalized sampling,  the investigation is quite limited. It remains open to answer what makes reverse diffusion different from conventional MCMC.
From our perspective, by employing a distribution parameterization $q_\theta$ for the formulation of $q_t$, a notable outcome is the acquisition of the ``learned'' posterior mean $\mu_\theta(\rvx)$, which can be perceived as analogous to the score function. This perspective grants us the opportunity to draw a connection between the denoising score matching loss employed in diffusion models, as outlined in the works of \citet{vincent2011connection} and \citet{ho2020denoising}, and the parameterization of the posterior mean. Such recognition allows us to comprehend the denoising score matching loss as a means of parameterizing the posterior mean within the context of diffusion models. Our proposed $q_t$ is the non-parametric version of denoising score matching, which is more suitable for posterior sampling tasks.~\xunp{We should present the connection and differences between score-based models and our methods. Their tasks are different, in score-based models samples are given while density unknown, in sampling tasks ....}

\subsection{Reverse Diffusion in Diffusion Models}
%\textcolor{blue}{Put the discussion of the diffusion models here (setup, OU processes, reverse process, discretization, etc.). Leave equation (3.1) out though.}

\noindent\textbf{Setup.} Given an OU process from $p_*$ to $\cN\left(\vzero,\mI\right)$, we expect to draw samples from $p_*$ with the reverse process.
Thus, we can track the random variable $\rvx$ at time $t$ with density function $p_t$, such that $p_0 = p_*$ and $p_\infty$ is the density of $\cN\left(\vzero,  \mI\right)$. For computation consideration, we focus on the $t\in[0,T]$.
At the sampling stage, we will consider the reverse stochastic differential equation from $[0,T]$, with random variable $\hat{\rvx}_t$ and the corresponding density function $\hat{p}_t$ such that $p_t = \hat{p}_{T-t}$. Considering the discretization error, we have $\bar{\rvx}_t$ and $\bar{p}_t$.
Besides, when taking score estimation into account, we use $\tilde{\rvx}_t^{p_T}$ and $\tilde{p}_t^{p_T}$ \xunp{(maybe we should simplify the notation here. We seem to only use $p$ and $\tilde{p}$ in our main text, and other notations can remove to appendix)}.
Also, when the starting distribution of the reverse process is $p_\infty$ rather than $p_T$, we use $\tilde{\rvx}_t$ and $\tilde{p}_t$. 
The capital $P$ denotes the law of the stochastic process (the joint distribution of the whole trajectory).
To make it more organized, we arrange the notations as Table~\ref{tab:notation_list}.

\noindent\textbf{Ideal reverse of OU process.}
Similar to the diffusion model, the OU process is chosen as follows
\begin{equation}
    \label{eq:ou_sde}
    \der \rvx_t = -\rvx_t \der t + \sqrt{2}\der B_t,\quad \rvx_0\sim p_0 \propto e^{-f_*},
\end{equation}
where $(B_t)_{t\ge 0}$ is Brownian motion in $\R^d$ and $p_0$ is assigned as $p_*$. 
%The OU process is a unique time-homogeneous Markov process which is also a Gaussian process.
The stationary distribution of \eqref{eq:ou_sde} is $p_\infty \propto \exp(-\frac{1}{2}\left\|\rvx\right\|^2)$.
According to \cite{cattiaux2021time}, under mild conditions in the following forward process
$
    \der \rvx_t = b_t(\rvx_t)\der t + \sqrt{2}\der B_t,
$
the reverse process also admits an SDE description. If we fix the terminal time $T>0$ and set
$
    \hat{\rvx}_t = \rvx_{T-t}, \quad \mathrm{for}\ t\in[0, T],
$
 the process $(\hat{\rvx}_t)_{t\in[0,T]}$ satisfies the SDE
$
    \der \hat{\rvx}_t = \hat{b}_t(\hat{\rvx}_t)\der t+ \sqrt{2} \der B_t,
$
where the reverse drift satisfies the relation
$
    b_t + \hat{b}_{T-t} = 2 \grad \ln p_t,  \rvx_t\sim p_t.$
In this condition, the reverse process of Eq.~\eqref{eq:ou_sde} is as follows
\begin{equation}
    \label{def:bw_sde}
   \der \hat{\rvx}_t = \left(\hat{\rvx}_t + 2\grad\ln p_{T-t}(\hat{\rvx}_t)\right)\der t +\sqrt{2} \der B_t.
\end{equation}
Thus, once the score function $\nabla\ln p_{T-t}$ is obtained, the reverse SDE induce a sampling algorithm.



\noindent\textbf{Discretization and realization of the reverse process. }
To obtain the particles along SDE ~\eqref{def:bw_sde}, the first step is to initialize the particle with a tractable starting distribution. 
In real practice, it is usually hard to sample from the ideal initialization $p_T$ directly due to its unknown properties.
Instead, we sample from an approximated distribution $\hat{p}$. For large $T$, $p_\infty$ is chosen for approximating $p_T$ as   their gap can be controlled. For the iteration, we utilize the numerical discretization method, i.e., DDPM~\cite{ho2020denoising}, widely used in diffusion models' literature.
Different from ULA, DDPM divides SDE \eqref{def:bw_sde} by different time segments, 
and consider the following SDE for each segment
\begin{equation}
    \label{sde:bps}
    \der \bar{\rvx}_t = \left(\bar{\rvx}_t + 2 \grad \ln p_{T-k \eta}(\bar{\rvx}_{k\eta})\right)\der t + \sqrt{2} \der B_t, \quad t\in\left[k\eta, (k+1)\eta\right],\quad \bar{\rvx}_0 \sim p_T
\end{equation}
to discretize SDE \eqref{def:bw_sde}.
%Therefore, we will formulate its SDE and solve the main difficulty\xunp{what does this sentence mean ?}.
%Similar to~\cite{ho2020denoising}, we divide SDE.~\ref{def:bw_sde} by different time segments. 
%For each segment, we consider the following SDE
%\begin{equation}
%    \label{sde:bps}
%    \der \bar{\rvx}_t = \left(\bar{\rvx}_t + 2 \grad \ln p_{T-k \eta}(\bar{\rvx}_{k\eta})\right)\der t + \sqrt{2} \der B_t, \quad t\in\left[k\eta, (k+1)\eta\right],\quad \bar{\rvx}_0 \sim p_T
%\end{equation}
%to approximate Eq.~\eqref{def:bw_sde}.
Suppose we obtain $\rvv_k$ to approximate $2\nabla\ln p_{T-k \eta}$ at each iteration.
Then, we are able to find the analytic solution of 
\begin{equation}
    \label{sde:readl_prac_bps}
    \der \tilde{\rvx}_t = \left(\tilde{\rvx}_t + \rvv_k(\tilde{\rvx}_{k\eta})\right)\der t + \sqrt{2} \der B_t, \quad t\in\left[k\eta, (k+1)\eta\right], \quad  \tilde{\rvx}_0\sim p_{\infty}.
\end{equation}
Specifically, by setting auxiliary random variable as $\rvr_i\left(\tilde{\rvx}_t,t\right)\coloneqq \tilde{\rvx}_{t,i} e^{-t}$, we have
\begin{equation*}
    \begin{aligned}
        \der \rvr_i(\tilde{\rvx}_t,t) = &\left(\frac{\partial \rvr_i}{\partial t} + \frac{\partial \rvr_i}{\partial \tilde{\rvx}_{t,i}}\cdot \left[\rvv_{k,i} + \tilde{\rvx}_{t,i}\right] +   \Tr \left(\frac{\partial^2 \rvr_i}{\partial \tilde{\rvx}_{t,i}^2}\right)\right)\der t + \frac{\partial \rvr_i}{\partial \tilde{\rvx}_{t,i}}\cdot \sqrt{2} \der B_t\\
      %  =& \left(-\tilde{\rvx}_{t,i} e^{-t} + e^{-t}\cdot \left(\rvv_{k,i}+\tilde{\rvx}_{t,i}\right)\right)\der t + e^{-t}\der B_t\\
        = & \rvv_{k,i}e^{-t}\der t + \sqrt{2} e^{-t}\der B_t,
    \end{aligned}
\end{equation*}
where the equalities are derived by the It\^o's Lemma.
Then, we set the initial value $\rvr_0(\tilde{\rvx}_t,0)=\tilde{\rvx}_{t,i}$, 
%\xunp{$\rvr_i(\tilde{\rvx}_t,0)=\tilde{\rvx}_{t,i}$ where $i$ denotes the coordinate.}
and integral on both sides of the equation. We have
\begin{equation}
    \label{eq:par_update}
    \begin{aligned}
         \tilde{\rvx}_{t+s} 
         = e^{s}\tilde{\rvx}_t + \left(e^{s}-1\right)\rvv_k + \mathcal{N}\left(0,  \left(e^{2s}-1\right)\mI_d\right),
    \end{aligned}
\end{equation}
where $\rvv_k$ is the score estimate.
Then, we construct $\rvv_k$ to approximate the true score function \xunp{(should we refer to the detailed section, i.e., Section~\ref{sec:score})}.

\iffalse
Specifically, for each time $t>0$,
    \begin{equation}\label{eq:convert}
    \begin{aligned}
        \grad_{\vx} \ln p_{t}(\vx) =  \mathbb{E}_{\rvx_0 \sim q_{t}}\left[\frac{  e^{-t}\rvx_0-\vx}{\left(1-e^{-2t}\right)}\right],\text{ s.t. } q_{t}(\vx_0|\vx)  \propto \exp\left(-f_{*}(\vx_0)-\frac{\left\|\vx - e^{-t}\vx_0\right\|^2}{2\left(1-e^{-2t}\right)}\right),
    \end{aligned}
\end{equation}
where $p_0(\vx)\propto\exp(-f_*(\vx))$.
The estimation of $\nabla \ln p_t$ can be accomplished by computing the mean of $q_t(\vx_0|\vx)$, as shown in Eq.~\eqref{eq:convert}. Here, $q_t(\vx_0|\vx)$ represents the posterior distribution of $\vx_0$ given $\vx$. Notably, the conditional probability of $q_t$ exhibits a simpler form compared to that of $p_0$, particularly in cases where $t$ is small. This simplicity arises from the inclusion of an additional quadratic term in the conditional probability of $q_t$. Consequently, the original sampling problem of drawing samples from $p_0$ can be effectively transformed into the task of sampling from $q_t$.
\fi










==> 0_contents/030algorithm_backup.tex <==
Therefore, we present a concise summary of our algorithm as follows:
\begin{enumerate}
    \item Determine a proper parameter $T$ such that the probability distribution $p_T$ closely approximates the limiting distribution $p_\infty$, and choose the step size $\eta$ of the backward process.
    \item Generate a sample from the limiting distribution $p_\infty$ as $\tilde{p}_0$.
    \item Sample from a distribution that effectively approximates the distribution $q_{T-k\eta}$ and construct the velocity $\rvv_k$ with Eq.~\eqref{eq:construction_of_v}.
    \item Update the sample using the generated velocity $\rvv_k$ and Eq.~\eqref{eq:par_update}.
    \item  Repeat steps (3) and (4) iteratively until the value of $k\eta$ closely approximates $T$.
\end{enumerate}



%--------------------- Section 3 backup
\section{The Reverse Diffusion Monte Carlo Approach}
%\textcolor{blue}{Move most of the setup, sec. 3.1, 3.2 into sec. 2.1. Focus on our contribution equation (3.1) here.}


%where $\vv_k$ is estimated by the following procedure.


%With this condition, to implement the particles' update, we estimate $\grad \ln p_{T-k \eta}(\tilde{\vx}_{k\eta})$ by $\vv_k$. Note that the starting distribution should also be a tractable one in real practice (such as $p_\infty$) rather than $p_T$.


\subsection{Score function from the posterior and rdMC algorithm}
\label{sec:score}


%Unlike generative modeling task, the unnormalized sampling 

\noindent\textbf{Computing score via mean estimation.} In generative modeling tasks, the score function is estimated by the true samples from $p_*$ with a noise corruption. However, in unnormalized sampling, samples from $p_*$ are unavailable. Fortunately, we found that the estimation is still feasible by sampling from a well-behaved distribution. The following Lemma describes the idea.
\begin{lemma} \label{lem:reform}
Assume that Eq.~\eqref{eq:ou_sde} and \eqref{def:bw_sde} define the forward and reverse process. Then the score function can be rewritten as
\begin{equation}
    \label{eq:grad_}
    \begin{aligned}
    \textstyle
        \grad_{\vx} \ln p_{T-t}(\vx) =  \mathbb{E}_{\vx_0 \sim q_{T-t}(\cdot|\vx)}\left[-\frac{\vx - e^{-(T-t)}\vx_0}{\left(1-e^{-2(T-t)}\right)}\right],
    \end{aligned}
\end{equation}
where the conditional density function is 
\begin{equation}
\textstyle
q_{T-t}(\vx_0|\vx)  \propto \exp\left(-f_{*}(\vx_0)-\frac{\left\|\vx - e^{-(T-t)}\vx_0\right\|^2}{2\left(1-e^{-2(T-t)}\right)}\right).
\label{eq:distribution_q}
\end{equation}
\end{lemma}

Lemma \ref{lem:reform} indicates that the score function of the OU process is the mean of the posterior $q_{T-t}(\cdot|\vx)$. Thus, we can sample from $q_{T-t}(\cdot|\vx)$ and estimate the score by empirical mean and perform the reverse SDE by discretization. 
In this condition, suppose $\tilde{\vx}_{k\eta}=\vx$ for any $\vx\in\R^d$, the construction of $\vv_k(\vx)$ in Eq.~\eqref{sde:readl_prac_bps} can be presented as
\begin{equation}
    \label{eq:construction_of_v}
    \textstyle
    \vv_k(\vx) = \frac{1}{n_k}\sum_{i=1}^{n_k}  \vv_k^{(i)}(\vx)\quad \mathrm{where}\quad \vv^{(i)}_k(\vx) =  2\left(1-e^{-2(T-k\eta)}\right)^{-1}\cdot \left(e^{-(T-k\eta)}{\vx^{(i)}_k} - \vx\right),
\end{equation}
the random variables satisfy $\vx_k^{(i)}\sim q_{T-k\eta}(\cdot|\vx)$ and $n_k$ denotes the sample number for controlling the gap between $\vv_k(\vx)$ and $\grad_{\vx} \ln p_{T-k\eta}(\vx)$.

Once the score function can be estimated, the sampling algorithm can be presented. The detailed algorithm is described in Algorithm~\ref{alg:bpsa}. By following these steps, our proposed algorithm efficiently addresses the given problem and demonstrates its effectiveness in practical applications.
Specifically, we summarize our algorithm as below: (1) choose proper $T$ and proper $\hat p$ such that $p_T\approx\hat p$. This step can be done by either $\hat p = p_\infty$ for large $T$ or performing the Langevin Monte Carlo for $p_T$; (2) sample from $\hat p$; (3) sample from a distribution that approximate $q_{T-t}$; (4) update $\tilde{p}_{t}$ with the approximated $q_{T-t}$ samples. This step can be done by Langevin Monte Carlo inner loop, as $\nabla\log q_{T-t}$ is explicit; (5) repeat (3) and (4) until $t\approx T$. After (5), we can also perform Langevin algorithm to fine-tune the steps when the gradient complexity limit is not reached. The main algorithm as Algorithm~\ref{alg:bpsa}.

%(Algorithm \ref{alg:initialization} in Appendix)


\begin{algorithm}[t]
    \caption{\textsc{rdMC}: reverse diffusion Monte Carlo }
    \label{alg:bpsa}
    \begin{algorithmic}[1]
            \STATE {\bfseries Input:} Initial particle $\tilde{\vx}_0$ sampled from $\hat{p}$, Terminal time $T$, Step size $\eta, \eta'$, Sample size $n$.%, Fine-grain iters $T_0$;
            \FOR{$k = 0$ to $\lfloor T/\eta \rfloor-1$}
                \STATE Set $\vv_k=\vzero$;
                \STATE Create $n$ Monte Carlo  samples to estimate $$\mathbb{E}_{\vx \sim q_{t}}\left[-\frac{\tilde{\vx}_{k\eta} - e^{-(T-k\eta)}\vx}{\left(1-e^{-2(T-k\eta)}\right)}\right],\text{ s.t. } q_{t}(\vx|\tilde{\vx}_{k\eta})  \propto \exp\left(-f_{*}(\vx)-\frac{\left\|\tilde{\vx}_{k\eta} - e^{-(T-k\eta)}\vx\right\|^2}{2\left(1-e^{-2(T-k\eta)}\right)}\right).$$
                \STATE Compute the corresponding estimator $\vv_k$.
                \STATE $\tilde{\vx}_{{(k+1)\eta}}=e^\eta\tilde{\vx}_{k\eta}+\left(e^\eta - 1\right)\vv_k +\xi \quad \text{where $\xi$ is sampled from }  \mathcal{N}\left(0,  \left(e^{2\eta}-1\right)\mI_d\right)$.
            \ENDFOR
            \iffalse
            \STATE $\vy_0 = \tilde{\vx}_{\lfloor T/\eta \rfloor \eta }$
            \FOR{$k = 0$ to $T_1-1$}
             \STATE $\vy_{k+1}=\vy_k-\eta'\nabla f_*(\vy_k) +\sqrt{2\eta'}\xi \quad \text{where $\xi$ is sampled from } \mathcal{N}\left(0,  \mI_d\right)$
            \ENDFOR
            \fi
            \STATE {\bfseries Return: $ \tilde{\vx}_{\lfloor T/\eta \rfloor \eta}$} .
    \end{algorithmic}
\end{algorithm}




In what follows, we will discuss the mean estimation task and 
describe several approaches.

%In an ideal scenario, the painless sampling of $q_t$ would yield the exact form of $\nabla\ln p_t$. However, in practical applications, the approximation of $q_t$ via sampling algorithms is often necessary. Notably, when $t$ is small, the strong convexity of $\ln q_t$ arises from the dominance of the quadratic term, thereby facilitating the sampling of $q_t$. 
%Conversely, for large $t$, the score approaches $\vx$ due to the proximity of $p_t$ to a Gaussian distribution. As a result, the dependence of the $q_t$ mean weakens, rendering a highly accurate approximation of $q_t$ unnecessary. The subsequent sections will delve into the underlying approximations of $q_t$.
\noindent\textbf{Sampling from $q_{T-t}(\cdot|\vx)$.}
The above paragraph describes the mean estimation formula of the score function $\grad_{\vx} \ln p_{T-t}(\vx)$, assuming one can generate samples from the conditional density function $q_{T-t}(\cdot|\vx)$.
In practice, we need a procedure to generate (approximate) samples from $q_{T-t}$.
% Although the sampling oracle of $q_{T-t}$ would yield the exact form of $\nabla\ln p_{T-t}$, the approximation of $q_{T-t}$ via sampling algorithms is often necessary in practice.
Before describing the specific procedure, we highlight some important properties of $q_{T-t}$.
\begin{itemize}
    \item When $t$ is close to $T$, the quadratic term of Eq.~\eqref{eq:distribution_q} dominates, making distribution $q_{T-t}(\cdot|\vx)$ strongly log-concave, and consequently easy to sample from. 
    \item When $t$ is close to $0$ in Eq.~\eqref{eq:grad_}, $e^{-(T-t)} \approx e^{-T}$ and becomes small for large $T$. 
    This renders the score estimation to dependence less on the samples $\vx_0$ from $q_{T-t}$, allowing for higher error tolerance when sampling from $q_{T-t}(\cdot|\vx)$.
    % the diminishing weight of mean estimation in Eq.~\eqref{eq:grad_} will be close to $e^{-T}$ and means a large error can be tolerated. As a result, the dependence of the $q_t$ mean weakens, rendering a highly accurate approximation of $q_{T-t}(\cdot|\vx)$ unnecessary.
\end{itemize}
By definition, $q_t$ is the posterior of the $\vx_0$, such that $q_t(\vx_0|\vx) = \frac{p_0(\vx_0) \cdot p_t(\vx|\vx_0)}{p_t(\vx)}.$  Moreover, we have the explicit score function for each $q_t$. Thus, we need to sample from $q_t$ as a sub-problem. We will introduce our solution as below. 

%\textcolor{red}{what are you trying to say in the above paragraph?}
%\textcolor{red}{Say something like ``We use ULA to sample from $q_{T-t}$. But there are issues with its computation complexity in the small $t$ case. Smart initialization may help...''}

\noindent\textbf{Importance weighted score estimator.}
In this paragraph, we consider an alternative importance sampling approach for estimating the score $\grad\ln p_{T-t}$.
From Eq.~\eqref{eq:grad_}, we know that the key is to estimate:
{\footnotesize
\begin{align*}
&\grad_{\vx} \ln p_{T-t}(\vx) 
= \mathbb{E}_{\vx_0 \sim q_{T-t}(\cdot|\vx)}\left[\frac{e^{-(T-t)}\vx_0 - \vx}{\left(1-e^{-2(T-t)}\right)}\right]
= \frac{1}{Z_*} \mathbb{E}_{\vx_0 \sim \rho_{T-t}(\cdot|\vx)}\left[\frac{ e^{-(T-t)}\vx_0-\vx }{\left(1-e^{-2(T-t)}\right)} \cdot e^{-f_*(\vx_0)}\right],
\end{align*}}
and
$$
Z_* = \mathbb{E}_{\vx_0 \sim \rho_{T-t}(\cdot|\vx)}\left[ \exp(-f_*(\vx_0))\right],
$$
% \begin{align*}
% &\EE_{p_{0}(\vx_0)} \left[e^{-\frac{\left\|\vx - e^{T-t}\vx_0\right\|^2}{2\left(1-e^{-2(T-t)}\right)}} \cdot \frac{  e^{-(T-t) }\vx_0-\vx}{\left(1-e^{-2(T-t)}\right)}\right] = \frac{1}{Z_*} \mathbb{E}_{\vx_0 \sim \rho_{T-t}(\cdot|\vx)}\left[\frac{ e^{-(T-t)}\vx_0-\vx }{\left(1-e^{-2(T-t)}\right)} \cdot e^{-f_*(\vx_0)}\right],
% \end{align*}
% and
% \begin{align*}
% \int_{\R^d} p_{0}(\vx_0)\cdot \exp\left(\frac{-\left\|\vx - e^{-(T-t)}\vx_0\right\|^2}{2\left(1-e^{-2(T-t)}\right)}\right)\der \vx_0
% = \frac{1}{Z_*} \mathbb{E}_{\vx_0 \sim \rho_{T-t}(\cdot|\vx)}\left[ \exp(-f_*(\vx_0))\right],
% \end{align*}
where 
$
\rho_{T-t}(\cdot|\vx) \propto \exp\left(\frac{-\left\|\vx - e^{-(T-t)}\vx_0\right\|^2}{2\left(1-e^{-2(T-t)}\right)}\right). 
$  Note that sampling from the normal distribution $\rho_{T-t}$ takes negligible computation resource.
The question is the sample complexity of estimating the two aforementioned expectations. %:$\mathbb{E}_{\vx_0 \sim \rho_{T-t}(\cdot|\vx)}\left[-\frac{\vx - e^{-(T-t)}\vx_0}{\left(1-e^{-2(T-t)}\right)} \cdot e^{-f_*(\vx_0)}\right]$ and $\mathbb{E}_{\vx_0 \sim \rho_{T-t}(\cdot|\vx)}[e^{-f_*(\vx_0)}]$
Since $\rho_{T-t}(\vx_0|\vx)$ is a Gaussian density with variance $\sigma_t^2 = \frac{1-e^{-2(T-t)}}{e^{-2(T-t)}}$, we know that as long as $-\frac{\vx - e^{-(T-t)}\vx_0}{\left(1-e^{-2(T-t)}\right)} \cdot \exp(-f_*(\vx_0))$ is a $G$-Lipschitz function, the sample complexity scales as $N=\tilde{O}\left({\sigma_t^2} \frac{G^2}{\epsilon^2} \right)$ for the resulting errors of the two mean estimators to be less than $\epsilon$~\citep{wainwright2019high}.

However, the sample size required of the importance sampling method to achieve an overall small error is known to scale exponentially with the KL divergence between $\rho_{T-t}$ and $q_{T-t}$~\citep{persi2018importancesampling}, which can depend on the dimension. 
In our current formulation, this is due to the fact that the true denominator $Z_*=\mathbb{E}_{\vx_0 \sim \rho_{T-t}(\cdot|\vx)}[e^{-f_*(\vx_0)}]$ can be as little as $\exp(-d)$. 
As a result, to make the overall score estimation error small, the error tolerance---and in turn the sample size---required for estimating $Z_*$ can scale exponentially with the dimension.

\noindent\textbf{ULA score estimator with importance sampling initialization.} 
To address the above mentioned issues, we combine the importance sampling approach with the unadjusted Langevin algorithm (ULA).
In particular, we first implement the importance sampling method to form a rough score estimator. We then initialize the ULA algorithm at the mean estimator and obtain a refined score estimate. 
Via this combination, we are able to efficiently obtain accurate score estimation by virtue of the ULA algorithm when $t$ is close to $T$. When $t$ is close to $0$, we are able to quickly obtain rough score estimates via the importance sampling approach.
We discover empirically that this combination generally perform well when $t$ interpolates the two regimes (Sec.~\ref{sec:exp}). 
%\textcolor{red}{Is this what you wanna describe?}
% To address the issues mentioned above, we consider that \( q_t \) can also be estimated by ULA. In this way, when \( \exp(-f_*(x)) \) is highly concentrated, we can use the gradient information from ULA for accurate estimation.
% Nonetheless, importance sampling can provide some insights for ULA as a good initialization. Therefore, in actual algorithms, we can combine the features of both, first using importance sampling to get a rough mean estimate, and then refining it with ULA to obtain an accurate score estimate. 
 
 %Thus, we can initialize with the importance samples and perform Langevin inner loop to approximate $q_{T-t}$ in real practice.
%In practice, due to the target distribution \( \exp(-f_*(x)) \) often being highly concentrated, it is difficult to estimate the true mean accurately using importance sampling.
%\paragraph{ULA inner loop estimator $\vv_t$ in  Alg~\ref{alg:bpsa}.}
%Suppose we require the final total variation less than $\epsilon$ and target distribution $p_*$ satisfies Assumption~\ref{ass:lips_score}-\ref{ass:curve_outside_ball} where $n>0$, and the KL divergence between $p_*$ the standard normal distribution is denoted as $C_0$. 

%\subsection{The rdMC Algorithm}



\subsection{Reverse SDE vs Langevin dynamics: Intuition}
From Figure \ref{fig:gmm_intro}, we observe that the \textsc{rdMC} method deviates significantly from the conventional gradient-based MCMC techniques, such as Langevin dynamics. 
In particular, Figure \ref{fig:gmm_intro} visualizes the paths from a Gaussian distribution to a mixture of Gaussian distributions. The first row represents the paths guided by Langevin dynamics, while the second row represents the paths guided by the reverse SDE. It can be observed that Langevin dynamics, being solely driven by the gradient information of the target density $p_*$, tends to get trapped in local regions, resulting in uneven sampling of the mixture of Gaussian distribution. 
From a theoretical point of view, $p_*$ admits a small log-Sobolev constant due to the separation of the modes \citep{ma2019sampling,schlichting2019poincare,menz2014poincare}. Consequently, the convergence of conventional MCMC methods becomes notably challenging in such scenarios \citep{tosh2014lower}.
In contrast, \textsc{rdMC} is unaffected by local gradients, enabling it to distribute samples more evenly across different modes. 
As a result, \textsc{rdMC} enjoys faster convergence in those challenging cases.
This intuition also explains why diffusion models excel in modeling complex distributions in high-dimensional spaces.  
%\textcolor{red}{Perhaps add a reference here?}




==> 0_contents/040_analysis_backup_june9.tex <==
\section{Reverse Diffusion Sampling}
In this section, we will discuss the properties of our algorithm. 
First, we compare the reverse SDE with Langevin dynamics by visualization when the target distribution satisfies good properties, e.g., log-concave or LSI.
It shows that, compared with Langevin dynamics, the reverse SDE makes the underlying distribution of particles closer to the target distribution $p_*$ in the same timestamp.
Then, under some mild assumptions, we provide the theoretical convergence of RDS without isoperimetry.
%In this section, we will discuss the properties of our algorithm, including the interpretation and the analysis. Particularly, our algorithm can support general distributions without isoperimetry thanks to the reverse SDE of the OU process.
\subsection{Reverse SDE vs Langevin dynamics}
Within this segment of our study, our aim is to present a set of illustrative examples that effectively showcase the profound effectiveness of the reverse SDE framework. It is imperative to highlight that this methodology deviates significantly from the conventional gradient-based MCMC techniques, such as Langevin dynamics. By offering intuitive examples, we strive to provide compelling evidence and foster a comprehensive understanding of the remarkable capabilities and advantages exhibited by reverse SDE in comparison to its gradient-based MCMC counterparts.

Figure \ref{fig:gaussian} demonstrate the differences between Langevin dynamics and the OU process in terms of their trajectories. The former utilizes the gradient information of the target distribution $\nabla\ln p_*$, to facilitate optimization. However, it converges slowly in directions with small gradients. On the other hand, the OU process constructs paths with equal velocities in each direction, thereby avoiding the influence of gradient vanishing directions. Consequently, leveraging the reverse process of the OU process is advantageous for addressing the issue of uneven gradient sampling across different directions.  Figure \ref{fig:gmm} visualizes the paths from a Gaussian distribution to a mixture of Gaussian distributions. The first row represents the paths guided by Langevin dynamics, while the second row represents the paths guided by the reverse SDE. It can be observed that Langevin dynamics, being solely driven by the gradient information of the target distribution $p_*$, tends to get trapped in local regions, resulting in uneven sampling of the mixture of Gaussian distribution. In contrast, the reverse SDE is unaffected by local gradients, enabling it to distribute samples more evenly across different modes. This is also why diffusion models excel in modeling complex distributions in high-dimensional spaces. It is worth emphasizing that both examples mentioned exhibit a common challenge characterized by a small log-Sobolev constant. Specifically, the presence of a large Gaussian variance direction and isolated modes within the mixture distributions result in a diminished log-Sobolev constant. Consequently, the convergence of conventional MCMC methods becomes notably challenging in such scenarios. In stark contrast, our proposed algorithm demonstrates robustness in handling these challenging cases and exhibits enhanced convergence properties.



\begin{figure}
    \centering
    \begin{tabular}{cccc}
          \includegraphics[width=3.15cm]{figs/x0.pdf} & \includegraphics[width=3.15cm]{figs/xopt.pdf} & 
          \includegraphics[width=3.15cm]{figs/forward.pdf} &
          \includegraphics[width=3.15cm]{figs/backward.pdf} \\
          $\mathcal{N}(0,\mI_d)$& $p_*$&Langevin $\mu_t$&OU process $\mu_t$
    \end{tabular}
    \caption{ Langevin dynamics vs (reverse) OU process. We consider the sampling path between $\mathcal{N}(0,\mI_2)$ and $\mathcal{N}([20,20],\operatorname{diag}(400,1))$.
    The mean $\mu_t$ of Langevin dynamics show varying convergence speeds in different directions, while the OU process demonstrates more uniform changes. }
    \label{fig:gaussian}
\end{figure}




\begin{figure}
    \centering
    \begin{tabular}{ccccc}
          \includegraphics[width=2.30cm]{figs/forward_0.pdf} & \includegraphics[width=2.30cm]{figs/forward_5.pdf} & 
          \includegraphics[width=2.30cm]{figs/forward_10.pdf} &
             \includegraphics[width=2.30cm]{figs/forward_1000.pdf} &
          \includegraphics[width=2.30cm]{figs/forward_10000.pdf} \\
          \includegraphics[width=2.30cm]{figs/backward_10000.pdf} &  
      \includegraphics[width=2.30cm]{figs/backward_1000.pdf} & \includegraphics[width=2.30cm]{figs/backward_200.pdf} & 
          \includegraphics[width=2.30cm]{figs/backward_100.pdf} &
          \includegraphics[width=2.30cm]{figs/backward_10.pdf} \\
    \end{tabular}
    \caption{ Langevin dynamics vs reverse SDE. The first and second rows depict the intermediate states of the Langevin algorithm and reverse SDE, respectively, illustrating the transition from $p_0$ to $p_*$. It can be observed that due to the local nature of $\ln p_*$ gradient information, the Langevin algorithm tends to get stuck in modes close to the initial state. In contrast, the reverse SDE excels at uniformly transporting particles to different modes. ($p_*$  is a Gaussian mixture distribution)}
    \label{fig:gmm}
\end{figure}


\subsection{Analysis}
\label{sec:analysis}
To provide the analysis of the convergence of RDS, we require the following assumptions.
\begin{enumerate}[label=\textbf{[\Subscript{A}{\arabic*}]}]
    \item \label{ass:lips_score} For all $t\ge 0$, the score $\grad \ln p_{t}$ is $L$-Lipschitz.
    \item \label{ass:second_moment} For some $\delta_0 >0$, $\mathbb{E}_{p_*}\left[\left\|\cdot\right\|^{2+\delta_0}\right]$ is finite. We also write $\mathbb{E}_{p_*}\left[\left\|\cdot\right\|^{2}\right]=m_2^2$ for the second moment of the target distribution $p_*$.
    \item \label{ass:curve_outside_ball} For any $\delta>0$, we can find some $R(\delta)$ satisfying $f_*(\vx)+\delta\left\|\vx\right\|^2$ is convex for $\left\|\vx\right\|\ge R(\delta)$. Without loss of generality, we suppose $R(\delta) = c_R/\delta^n$ for some $n>0,c_R>0$.
    %\label{ass:curve_outside_ball} For any $\delta>0$, we can find some $R(\delta)$ satisfying $\grad^2 f_*(\vx)\succeq -\delta \mI$ when $\left\|\vx\right\|\ge R(\delta)$.
\end{enumerate}

Assumption \ref{ass:lips_score} plays a pivotal role in governing the smoothness characteristics of the forward process. By imposing certain constraints on the Lipschitz continuity of the score function, the assumption ensures a well-behaved and predictable behavior of the process.
In addition, Assumption \ref{ass:second_moment} introduces essential constraints on the moments of the target distribution. These constraints effectively prevent an excessive accumulation of probability mass in the tail region, thereby ensuring a more balanced and well-distributed target distribution. 
It should be noted that the first two assumptions are also introduced in diffusion analysis~\cite{chen2022sampling}. Besides, \ref{ass:lips_score} can be released to the smoothness of $p_0$ with more sophisticated techniques \citep{chen2022improved}.

\paragraph{Beyond isoperimetry with Assumption~\ref{ass:curve_outside_ball}.}
Instead of requiring the isoperimetry in most previous analysis~\cite{vempala2019rapid,ma2021there}, we introduce~\ref{ass:curve_outside_ball} to analyze RDS convergence in a more general class of target distributions.
Intuitively, it allows the negative log density, i.e., $f_*$, to have a slow growth rate beyond some balls, which also implies the tail of $p_*$ can be heavier.
According to Proposition 5.4.1 in~\cite{bakry2014analysis}, if $p_*$ satisfies LSI, there exists some $\sigma>0$ which makes the following inequality 
\begin{equation}
    \label{ineq:lsi_crit}
    \int \exp\left(-f_*(\vx)+\frac{\sigma^2}{2}\left\|\vx\right\|^2\right)\der \vx <\infty
\end{equation}
establish. 
Actually, it is equivalent to requiring a quadratic growth of $f_*$ outside a ball, which would obviously be covered by~\ref{ass:curve_outside_ball}.
Besides, to make $p_*$ satisfy Poincar\'e inequality,~\citet{bakry2008simple} demonstrated that a sufficient condition is to make the following inequality 
\begin{equation}
    \label{ineq:poincare_crit}
    \left<\vx, \grad f_*(\vx)\right> \ge a\left\|\vx\right\|\quad \mathrm{s.t.}\ \left\|\vx\right\|\ge R
\end{equation}
hold for some $a, R>0$. 
The previous assumption fails when the growth of $f_*$ is slower than the linear function. 
If we consider a $1$-d distribution whose density function is
\begin{equation*}
    p_*(x)\propto \exp\left(-\left(x^2+1\right)^{1/4}\right).
\end{equation*}
We know $p_*$ has a bounded second moment, and its negative density function satisfies
\begin{equation*}
    \left|\grad^2 f_*(x)\right|=\left|\frac{1}{4}\cdot (2-x^2)\cdot \left(x^2+1\right)^{-7/4}\right|\le \frac{1}{2}.
\end{equation*}
However, due to its properties in the tail, $p_*$ will definitely violate Eq.~\ref{ineq:lsi_crit} and Eq.~\ref{ineq:poincare_crit}, which means it is hardly satisfied log-Sobolev or Poincar\'e inequality. 
However, it can be proved that $p_*$ satisfies Assumption~\ref{ass:curve_outside_ball}, whose detailed proof is deferred in Appendix~\ref{sec:app_nota_ass}.

These three assumptions collectively provide a robust theoretical framework that guarantees the desirable properties of the underlying distributions involved in sampling problems. The careful consideration and incorporation of these assumptions contribute to the overall effectiveness and reliability of the proposed approach.

\subsection{Inexact $q_t$ approximation}

In practical scenarios, obtaining the oracle sampler for $q_t$ is often challenging. However, since the density of $q_t$ is known, we can estimate its mean using sampling methods. 
To guarantee the convergence of RDS from a theoretical perspective, we provide a detailed implementation of Step 5 in Alg~\ref{alg:bpsa} in the following.
However, due to the difficulty of sampling beyond isoperimetry, the convergence rate we provided may not fully characterize the practical behavior. 
More empirical results can be found in our Appendix.

\paragraph{Implementation of Step 5 in Alg~\ref{alg:bpsa}}
Suppose we require the final total variation to be smaller than $\epsilon$, target distribution $p_*$ satisfies Assumption~\ref{ass:lips_score}-\ref{ass:curve_outside_ball} where $n>0$, and the KL divergence between $p_*$ and the normal distribution is denoted as $C_0$. 
With the following settings
\begin{small}
\begin{equation*}
    \begin{aligned}
        &\hat{\epsilon} = \exp\left(-32L\cdot 36^n \epsilon^{-8n}\right)\le \epsilon,\quad  \eta= C_1 (d+m_2^2)^{-1}\hat{\epsilon}^2,\quad a= \min\left\{2, -\frac{1}{2n}\log_{\epsilon}\left(\frac{-\ln \epsilon}{32L\cdot 36^n}\right)\right\}, \\
        &C_1 =2^{-9}\cdot 3^{-3}L^{-2},\quad C_2 =2^{-9}\cdot C_1^6 C_0^{-1},\quad C_3=2^{-20}C_0^{-2}C_1^{4},\quad \tilde{C}_{\mathrm{LSI}}= \frac{1}{6} \exp\left(-16\left(L+1\right)R^2\left(\frac{1}{6}\right)\right),\\
        & \tilde{q}_{T-k\eta}(\vx_0|\vx) \propto \exp\left(-f_*(\vx_0)- \frac{1}{2} \left\|\vx_0\right\|^2+\frac{e^{-(T-k\eta)}}{1-e^{-2(T-k\eta)}}\vx_0^\top \vx\right), 
    \end{aligned}
\end{equation*}
\end{small}

we divide the Alg~\ref{alg:bpsa} into four stages. 
For each stage, Step 5 conducts a ULA whose settings are shown in the following table.
\begin{table*}[!hbtp]
    \scriptsize
    \centering
    \begin{tabular}{ccccc}
    \toprule
     Stage & Target & Step size & Iteration number & Sample number ($n_k$) \\
     \midrule
     $e^{-2(T-k\eta)}\leq \hat{\epsilon}^2$ & $\tilde{q}_{T-k\eta}(\cdot|\vx)$ & $\frac{\tilde{C}_{ \mathrm{LSI} } C_2 \hat{\epsilon}^{20}}{16(L+1)^2 d (d+m_2^2)^8}$  & $\frac{320(L+1)^2d(d+m_2^2)^9}{C_2\tilde{C}^2_{\mathrm{LSI}}\hat{\epsilon}^{21}}$ & $\frac{16(d+m_2^2)^3}{C_1^2\hat{\epsilon}^6}$\\
     \midrule
     $\hat{\epsilon}^2<e^{-2(T-k\eta)}\leq \hat{\epsilon}^a$ & $\tilde{q}_{T-k\eta}(\cdot|\vx)$ & $\frac{\tilde{C}_{ \mathrm{LSI} } C_2 \hat{\epsilon}^{20}}{16(L+1)^2 d (d+m_2^2)^8}$ & $\frac{320(L+1)^2d(d+m_2^2)^9}{C_2\tilde{C}^2_{\mathrm{LSI}}\hat{\epsilon}^{21}}$ & $\frac{16(d+m_2^2)^3}{C_1^2\hat{\epsilon}^6}$\\
     \midrule
     $\hat{\epsilon}^a<e^{-2(T-k\eta)}\leq \frac{2L}{1+2L}$ & ${q}_{T-k\eta}(\cdot|\vx)$ & $\frac{C_{ \mathrm{LSI},k } C_3 \hat{\epsilon}^{26}}{64L^2 d (d+m_2^2)^6}$ & $\frac{2^{11}\cdot 3^2\cdot 13 L^2 d(d+m_2^2)^7}{C_3\hat{\epsilon}^{33}} $ & $\frac{2^9 C_0^{1/2}(d+m_2^2)^2}{C_1\hat{\epsilon}^9}$ \\
     \midrule
     $\frac{2L}{1+2L}\le e^{-2(T-k\eta)}< 1$ & ${q}_{T-k\eta}(\cdot|\vx)$ & $\frac{C_2e^{2(T-k\eta)}(1-e^{-2(T-k\eta)})}{72d(d+m_2^2)^8\hat{\epsilon}^{-20}}$ & $\frac{320(L+1)^2d(d+m_2^2)^9}{C_2\tilde{C}^2_{\mathrm{LSI}}\hat{\epsilon}^{21}}$ & $\frac{16(d+m_2^2)^3}{C_1^2\hat{\epsilon}^6}$ \\
     \bottomrule
\end{tabular}
\end{table*}
With such an implementation of Step 5, we may have the following convergence of Alg~\ref{alg:bpsa}.
Due to the space limitation, we defer the proof in Appendix~\ref{sec:main_proof_app}.
\begin{theorem}
    \label{thm:main_con}
    If the OU process induced by $p_*$ satisfies Assumption \ref{ass:lips_score}, \ref{ass:second_moment}, \ref{ass:curve_outside_ball_app}. By performing Algorithm \ref{alg:bpsa}, with a probability at least $1-\epsilon$ by requiring a $\Omega\left(d^{16}\exp\left(1440L\cdot 36^{n}\epsilon^{-8n}\right)\right)$
gradient complexity.
We have  $\TVD\left(\tilde{p}_t, p_*\right) \le  \tilde{O}(\epsilon)$.
\end{theorem}

\section{Example}


\section{Alternative method for score estimation}
From Eq.~\eqref{eq:grad_}, we know that the key is to estimate the following integrals up to the common constant $Z_*$ that will be canceled out:
\begin{align*}
&\int_{\R^d} p_{0}(\vx_0) \cdot \exp\left(\frac{-\left\|\vx - e^{T-t}\vx_0\right\|^2}{2\left(1-e^{-2(T-t)}\right)}\right) \cdot \left(-\frac{\vx - e^{-(T-t) }\vx_0}{\left(1-e^{-2(T-t)}\right)}\right)\der \vx_0 \\
&= \frac{1}{Z_*} \mathbb{E}_{\rvx_0 \sim \rho_{T-t}(\cdot|\vx)}\left[-\frac{\vx - e^{-(T-t)}\rvx_0}{\left(1-e^{-2(T-t)}\right)} \cdot \exp(-f_*(\vx_0))\right],
\end{align*}
and
\begin{align*}
\int_{\R^d} p_{0}(\vx_0)\cdot \exp\left(\frac{-\left\|\vx - e^{-(T-t)}\vx_0\right\|^2}{2\left(1-e^{-2(T-t)}\right)}\right)\der \vx_0
= \frac{1}{Z_*} \mathbb{E}_{\rvx_0 \sim \rho_{T-t}(\cdot|\vx)}\left[ \exp(-f_*(\vx_0))\right],
\end{align*}
where 
\[
\rho_{T-t}(\cdot|\vx) \propto \exp\left(\frac{-\left\|\vx - e^{-(T-t)}\vx_0\right\|^2}{2\left(1-e^{-2(T-t)}\right)}\right).
\]
Density $\rho_{T-t}$ can be trivially sampled from. 
The question is the sample complexity of estimating the two expectations:
$\mathbb{E}_{\rvx_0 \sim \rho_{T-t}(\cdot|\vx)}\left[-\frac{\vx - e^{-(T-t)}\rvx_0}{\left(1-e^{-2(T-t)}\right)} \cdot \exp(-f_*(\vx_0))\right]$ 
and $\mathbb{E}_{\rvx_0 \sim \rho_{T-t}(\cdot|\vx)}\left[ \exp(-f_*(\vx_0))\right]$.
Since $\rho_{T-t}(\rvx_0|\vx)$ is a Gaussian density with variance $\sigma^2 = \frac{1-e^{-2(T-t)}}{e^{-2(T-t)}}$, we know that as long as $-\frac{\vx - e^{-(T-t)}\rvx_0}{\left(1-e^{-2(T-t)}\right)} \cdot \exp(-f_*(\vx_0))$ is a $G$-Lipschitz function, the sample complexity scale as $N=\mathcal{O}\left({\sigma^2} \frac{G^2}{\epsilon^2} \right)$ (see e.g., Theorem 3.16 of Martin Wainwright's book ``High-dimensional statistics'').

This Lipschitzness seems to be a mild assumption on $f_*(\vx_0)$.

\subsection{How small is the denominator?}
Assume that we have aligned the functions so that $\min_{x_0} f_*(x_0) \approx 0$.
Also assume that function $f_*$ is $L$-Lipschitz smooth.
Then $\exp(-f_*(x_0)) \geq \exp\left( -\frac{L}{2} \left\| x_0-x_0^* \right\|^2 \right)$.
Therefore, 
\begin{align*}
\mathbb{E}_{\rvx_0 \sim \rho_{T-t}(\cdot|\vx)}\left[ \exp(-f_*(\vx_0))\right]
&\geq \frac{ \int \exp\left( -\frac{\left\|\vx - e^{-(T-t)}\vx_0\right\|^2}{2\left(1-e^{-2(T-t)}\right)} -\frac{L}{2} \left\| x_0-x_0^* \right\|^2 \right) \rd x_0 }{ \int \exp\left( -\frac{\left\|\vx - e^{-(T-t)}\vx_0\right\|^2}{2\left(1-e^{-2(T-t)}\right)} \right) \rd x_0 } \\
&= \left( \frac{\alpha}{\alpha+L} \right)^{d/2} \exp\left( - \frac{1}{2} \frac{\alpha L}{\alpha+L} \left\| e^{T-t} x - x_0^* \right\|^2 \right).
\end{align*}
where $\alpha = \frac{e^{-2(T-t)}}{1-e^{-2(T-t)}}$, and the last equality is obtain via completing the squares:
\begin{align*}
\frac{\left\|\vx - e^{-(T-t)}\vx_0\right\|^2}{\left(1-e^{-2(T-t)}\right)} + L \left\| x_0-x_0^* \right\|^2
= (\alpha+L) \left\| x_0 - \frac{\alpha e^{T-t}x + L x_0^*}{\alpha+L} \right\|^2
+ \frac{\alpha L}{\alpha+L} \left\| e^{T-t} x - x_0^* \right\|^2.
\end{align*}
We note that when $T-t$ is large, $\alpha$ is exponentially small.
Hence $\frac{\alpha}{\alpha + L} \approx \frac{\alpha}{L} \approx \frac{e^{-2(T-t)}}{L}$ and $\frac{\alpha L}{\alpha + L} \approx e^{-2(T-t)}$.
Therefore,
\[
\mathbb{E}_{\rvx_0 \sim \rho_{T-t}(\cdot|\vx)}\left[ \exp(-f_*(\vx_0))\right]
\gtrsim L^{-d/2} \cdot e^{-d(T-t)} \cdot e^{ -\frac{1}{2} \left\| x-e^{-(T-t)}x_0^* \right\|^2 }.
\]

==> 0_contents/040analysis_backup.tex <==
\section{Reverse Diffusion Sampling}
In this section, we will discuss the properties of our algorithm. 
First, we compare the reverse SDE with Langevin dynamics by visualization when the target distribution satisfies good properties,e.g., strongly log concave and LSI.
It shows that, compared with Langevin dynamics, the reverse SDE makes the underlying distribution of particles closer to the target distribution $p_*$ in the same timestamp.
Then, under some mild assumptions, we provide the theoretical convergence of RDS without isoperimetry.
%In this section, we will discuss the properties of our algorithm, including the interpretation and the analysis. Particularly, our algorithm can support general distributions without isoperimetry thanks to the reverse SDE of the OU process.
\subsection{Reverse SDE vs Langevin dynamics}
Within this segment of our study, our aim is to present a set of illustrative examples that effectively showcase the profound effectiveness of the reverse SDE framework. It is imperative to highlight that this methodology deviates significantly from the conventional gradient-based MCMC techniques, such as Langevin dynamics. By offering intuitive examples, we strive to provide compelling evidence and foster a comprehensive understanding of the remarkable capabilities and advantages exhibited by reverse SDE in comparison to its gradient-based MCMC counterparts.

Figure \ref{fig:gaussian} demonstrate the differences between Langevin dynamics and the OU process in terms of their trajectories. The former utilizes the gradient information of the target distribution $\nabla\ln p_*$, to facilitate optimization. However, it converges slowly in directions with small gradients. On the other hand, the OU process constructs paths with equal velocities in each direction, thereby avoiding the influence of gradient vanishing directions. Consequently, leveraging the reverse process of the OU process is advantageous for addressing the issue of uneven gradient sampling across different directions.


Figure \ref{fig:gmm} visualizes the paths from a Gaussian distribution to a mixture of Gaussian distributions. The first row represents the paths guided by Langevin dynamics, while the second row represents the paths guided by the reverse SDE. It can be observed that Langevin dynamics, being solely driven by the gradient information of the target distribution $p_*$, tends to get trapped in local regions, resulting in uneven sampling of the mixture of Gaussian distribution. In contrast, the reverse SDE is unaffected by local gradients, enabling it to distribute samples more evenly across different modes. This is also why diffusion models excel in modeling complex distributions in high-dimensional spaces.



\begin{figure}
    \centering
    \begin{tabular}{cccc}
          \includegraphics[width=3.15cm]{figs/x0.pdf} & \includegraphics[width=3.15cm]{figs/xopt.pdf} & 
          \includegraphics[width=3.15cm]{figs/forward.pdf} &
          \includegraphics[width=3.15cm]{figs/backward.pdf} \\
          $\mathcal{N}(0,I)$& $p_*$&Langevin $\mu_t$&OU process $\mu_t$
    \end{tabular}
    \caption{ Langevin dynamics vs (reverse) OU process. We consider the sampling path between $\mathcal{N}(0,I)$ and $\mathcal{N}([20,20],\operatorname{diag}(400,1))$.
    The mean $\mu_t$ of Langevin dynamics show varying convergence speeds in different directions, while the OU process demonstrates more uniform changes. }
    \label{fig:gaussian}
\end{figure}




\begin{figure}
    \centering
    \begin{tabular}{ccccc}
          \includegraphics[width=2.30cm]{figs/forward_0.pdf} & \includegraphics[width=2.30cm]{figs/forward_5.pdf} & 
          \includegraphics[width=2.30cm]{figs/forward_10.pdf} &
             \includegraphics[width=2.30cm]{figs/forward_1000.pdf} &
          \includegraphics[width=2.30cm]{figs/forward_10000.pdf} \\
          \includegraphics[width=2.30cm]{figs/backward_10000.pdf} &  
      \includegraphics[width=2.30cm]{figs/backward_1000.pdf} & \includegraphics[width=2.30cm]{figs/backward_200.pdf} & 
          \includegraphics[width=2.30cm]{figs/backward_100.pdf} &
          \includegraphics[width=2.30cm]{figs/backward_10.pdf} \\
    \end{tabular}
    \caption{ Langevin dynamics vs reverse SDE. The first and second rows depict the intermediate states of the Langevin algorithm and reverse SDE, respectively, llustrating the transition from $p_0$ to $p_*$. It can be observed that due to the local nature of $\ln p_*$ gradient information, the Langevin algorithm tends to get stuck in modes close to the initial state. In contrast, the reverse SDE excels at uniformly transporting particles to different modes. ($p_*$  is a Gaussian mixture distribution)}
    \label{fig:gmm}
\end{figure}


\subsection{Analysis}

To provide the analysis of the convergence of RDS, we require the following assumptions.
\begin{enumerate}[label=\textbf{[\Subscript{A}{\arabic*}]}]
    \item \label{ass:lips_score} For all $t\ge 0$, the score $\grad \ln p_{t}$ is $L$-Lipschitz.
    \item \label{ass:second_moment} For some $\delta_0 >0$, $\mathbb{E}_{p_*}\left[\left\|\cdot\right\|^{2+\delta_0}\right]$ is finite. We also write $\mathbb{E}_{p_*}\left[\left\|\cdot\right\|^{2}\right]=m_2^2$ for the second moment of the target distribution $p_*$.
    \item \label{ass:curve_outside_ball_app} For any $\delta>0$, we can find some $R(\delta)$ satisfying $f_*(\vx)+\delta\left\|\vx\right\|^2$ is convex for $\left\|\vx\right\|\ge R(\delta)$. Without loss of generality, we suppose $R(\delta) = c_R\delta^n$ for some $n>0,c_R>0$.
    %\label{ass:curve_outside_ball} For any $\delta>0$, we can find some $R(\delta)$ satisfying $\grad^2 f_*(\vx)\succeq -\delta \mI$ when $\left\|\vx\right\|\ge R(\delta)$.
\end{enumerate}

Assumption \ref{ass:lips_score} plays a pivotal role in governing the smoothness characteristics of the forward process. By imposing certain constraints on the Lipschitz continuity of the score function, the assumption ensures a well-behaved and predictable behavior of the process.
In addition, Assumption \ref{ass:second_moment} introduces essential constraints on the moments of the target distribution. These constraints effectively prevent an excessive accumulation of probability mass in the tail region, thereby ensuring a more balanced and well-distributed target distribution. 
It should be noted that the first two assumptions are also introduced in diffusion analysis~\cite{chen2022sampling}.

Different from the requirement of isoperimetry in most previous analysis,

\textcolor{blue}{\hrule}

Furthermore, Assumption \ref{ass:curve_outside_ball_app} imposes limitations on the tail behavior of the distribution, specifically targeting the avoidance of large negative curvatures. By constraining the growth of the distribution's tail, this assumption enhances the stability of the process. These three assumptions collectively provide a robust theoretical framework that guarantees the desirable properties of the underlying distributions involved in sampling problems. The careful consideration and incorporation of these assumptions contribute to the overall effectiveness and reliability of the proposed approach.

By using data-processing inequality, triangle inequality of total variation, and Pinsker's inequality,  we have 
\begin{equation}
    \label{ineq:main}
    \begin{aligned}
        \TVD\left(\tilde{p}_T, p_*\right) \le  \underbrace{\sqrt{\frac{1}{2}\KL\left(p_T\|p_\infty\right)}}_{\mathrm{Term\ 1}} + \underbrace{\sqrt{\frac{1}{2}\KL\left(\hat{P}_T \big\| \tilde{P}_{T}^{p_T}\right)}}_{\mathrm{Term\ 2}},
    \end{aligned}
\end{equation}
where the total variation distance to the target distribution can be controlled by two parts.

\begin{equation}
    \mathrm{Term\ 1} = \sqrt{\frac{1}{2}\exp\left(-\frac{T}{2}\right)\KL\left(p_0\| p_\infty\right)}
\end{equation}

\begin{equation}
    \label{ineq:term2_def}
    \begin{aligned}
        \mathrm{Term\ 2} = \sum_{k=0}^{N-1}\int_{k\eta}^{(k+1)\eta}\mathbb{E}_{\hat{P}_T}\left[\frac{1}{4}\cdot \left\|\rvv_k(\rvx_{k\eta}) - 2\grad\ln p_{T-t}(\rvx_t)  \right\|^2  \right] \der t. 
    \end{aligned}
\end{equation}

It is important to note that \textrm{Term 1} quantifies the proximity between the probability distributions $p_T$ and $p_\infty$. When selecting a value for the parameter $T$ that scales as $\mathcal{O}(\ln \frac{1}{\epsilon^2})$, we can establish that $\mathrm{Term\ 1}=\gO(\epsilon)$. The significance of \textrm{Term 2} lies in its representation of the KL divergence between the forward and backward trajectories, which corresponds to the mean squared error (MSE) of the induced drift force scores. By employing a small learning rate $\eta$ and effectively estimating $\nabla\ln p_{T-t}$, precise control over the MSE throughout the trajectory can be achieved.





\subsection{Oracle $q_t$}


Upon meticulous examination of the formulation for $q_t(\rvx_0|x)$, it becomes evident that it bears resemblance to a refined manifestation of the restricted Gaussian oracle (RGO) for $f_*$, as expounded in the early work \cite{lee2021structured}. Thus, when we can sample from the RGO problem, the reverse SDE can be estimated by finite particles.


\begin{proposition} If we possess an oracle sampler, denoted as $q_{T-t}$ where $t$ belongs to the interval $[0,T)$, and the sampler requires a number of samples on the order of $O(1/\epsilon^2)$ in each iteration, coupled with the update of particles from $p_\infty$ over a duration of XX iterations, it can be obtained that the total variation distance $\TVD\left(\tilde{p}_T, p\right)<\epsilon$.
\end{proposition}


\subsection{Inexact $q_t$ approximation}


In practical scenarios, obtaining the oracle sampler for $q_t$ is often challenging. However, since the density of $q_t$ is known, we can estimate its mean using sampling methods. To improve the efficiency of sampling, we partition the entire OU process into multiple stages, thereby reducing the number of gradient queries.

\noindent\textbf{Stage 1.} $e^{-2(T-k\eta)}\leq \epsilon^2$

\noindent\textbf{Stage 2.} $\epsilon^2<e^{-2(T-k\eta)}\leq \epsilon^a$, where $a=\min\left\{2, -\frac{1}{2n}\log_{\epsilon}\left(\frac{-\ln \epsilon}{32L\cdot 36^n}\right)\right\}$

\noindent\textbf{Stage 3.} $\epsilon^a<e^{-2(T-k\eta)}\leq \epsilon^a$.

\noindent\textbf{Stage 4.}

\begin{theorem}
    If the OU process induced by $p_*$ satisfis Assumption \ref{ass:lips_score}, \ref{ass:second_moment}, \ref{ass:curve_outside_ball_app}. By performing Algorithm \ref{alg:bpsa}, with a probability at least $1-\epsilon$ by requiring a $\Omega\left(d^{13}\exp\left(1440L\cdot 36^{n}\epsilon^{-8n}\right)\right)$
gradient complexity.
We have  $\TVD\left(\tilde{p}_t, p_*\right) \le  \tilde{O}(\epsilon).$
\xunp{Here, we may use $C$ to replace the detailed constant (and denote $C$ is independent to $d$ and $\epsilon$), and say you may find the constant $C$ in our appendix}

\end{theorem}


By using data-processing inequality, triangle inequality of total variation, and Pinsker's inequality,  we have 
\begin{equation}
    \label{ineq:main}
    \begin{aligned}
        \TVD\left(\tilde{p}_T, p_*\right) \le  \underbrace{\sqrt{\frac{1}{2}\KL\left(p_T\|p_\infty\right)}}_{\mathrm{Term\ 1}} + \underbrace{\sqrt{\frac{1}{2}\KL\left(\hat{P}_T \big\| \tilde{P}_{T}^{p_T}\right)}}_{\mathrm{Term\ 2}},
    \end{aligned}
\end{equation}
where the total variation distance to the target distribution can be controlled by two parts.

\begin{equation}
    \mathrm{Term\ 1} = \sqrt{\frac{1}{2}\exp\left(-\frac{T}{2}\right)\KL\left(p_0\| p_\infty\right)}
\end{equation}

\begin{equation}
    \label{ineq:term2_def}
    \begin{aligned}
        \mathrm{Term\ 2} = \sum_{k=0}^{N-1}\int_{k\eta}^{(k+1)\eta}\mathbb{E}_{\hat{P}_T}\left[\frac{1}{4}\cdot \left\|\rvv_k(\rvx_{k\eta}) - 2\grad\ln p_{T-t}(\rvx_t)  \right\|^2  \right] \der t. 
    \end{aligned}
\end{equation}

It is important to note that \textrm{Term 1} quantifies the proximity between the probability distributions $p_T$ and $p_\infty$. When selecting a value for the parameter $T$ that scales as $\mathcal{O}(\ln \frac{1}{\epsilon^2})$, we can establish that $\mathrm{Term\ 1}=\gO(\epsilon)$. The significance of \textrm{Term 2} lies in its representation of the KL divergence between the forward and backward trajectories, which corresponds to the mean squared error (MSE) of the induced drift force scores. By employing a small learning rate $\eta$ and effectively estimating $\nabla\ln p_{T-t}$, precise control over the MSE throughout the trajectory can be achieved.


%------------------backup 0928

\section{Analyses and Examples of the rdMC Approach}
\label{sec:exp}
%In this section, we will discuss the properties of our algorithm. 
%First, we compare the reverse SDE with Langevin dynamics by visualization when the target distribution satisfies good properties, e.g., log-concave or LSI.
%It shows that, compared with Langevin dynamics, the reverse SDE makes the underlying distribution of particles closer to the target distribution $p_*$ in the same timestamp.
%Then, under some mild assumptions, we provide the theoretical convergence of \textsc{rdMC} without isoperimetry.
%In this section, we will discuss the properties of our algorithm, including the interpretation and the analysis. Particularly, our algorithm can support general distributions without isoperimetry thanks to the reverse SDE of the OU process.

In this section, we focus on analyzing the overall complexity of the \textsc{rdMC} via ULA inner loop estimation.
The complexity of the importance sampling approach was described in Sec.\ref{sec:score}. \xunp{add some description about how to organize this section.}


To provide the analysis of the convergence of \textsc{rdMC}, we require the following assumptions.
\begin{enumerate}[label=\textbf{[\Subscript{A}{\arabic*}]}]
    \item \label{ass:lips_score} For all $t\ge 0$, the score $\grad \ln p_{t}$ is $L$-Lipschitz.
    \item \label{ass:second_moment} The second moment of the target distribution $p_*$ is upper bounded, i.e., $\mathbb{E}_{p_*}\left[\left\|\cdot\right\|^{2}\right]=m_2^2$.
    %\item \label{ass:convex_outside_ball} There exists $R>0$, such that  $f_*(\vx)$ is $m$-strongly convex when $\Vert \vx\Vert\geq R$.
    %\item \label{ass:curve_outside_ball} For any $r>0$, we can find some $R(r)$ satisfying $f_*(\vx)+r\left\|\vx\right\|^2$ is convex for $\left\|\vx\right\|\ge R(r)$. Without loss of generality, we suppose $R(r) = c_R/r^n$ for some $n>0,c_R>0$.
    %\label{ass:curve_outside_ball} For any $\delta>0$, we can find some $R(\delta)$ satisfying $\grad^2 f_*(\vx)\succeq -\delta \mI$ when $\left\|\vx\right\|\ge R(\delta)$.
\end{enumerate}

%\begin{enumerate}[label=\textbf{[\Subscript{$\tilde{\text{A}}$}{\arabic*}]}]
%  \setcounter{enumi}{2}
%  \item There exists $0<T\leq \frac{1}{2}\log\left(1+\frac{1}{2L}\right)$, such that $p_T$ is log-Sobolev with a constant  $C_T$, where $L$ is the constant in \ref{ass:lips_score}.
%\end{enumerate}

%\item \label{ass:curve_outside_ball_v2} For any $\delta>0$, we can find some $R(r)$ satisfying $f_*(\vx)+\delta\left\|\vx\right\|^2$ is convex for $\left\|\vx\right\|\ge R(r)$, such that $R(r) = \min\left\{c_R\ln\left(\frac{1}{r}\right),C_R\right\}$ for some $c_R,C_R>0$.
These assumptions are widely introduced in diffusion analysis, e.g., ~\cite{chen2022sampling}.
Specifically, Assumption \ref{ass:lips_score} governs the smoothness characteristics of the forward process, which ensure the feasibility of numerical discretization methods used for approximating the solution of continuous SDE.
Actually, this assumption can be alleviated by only requiring the smoothness of $p_* = p_0$ through \citep{chen2023improved} whose techniques are omitted in this paper to make our analysis clearer.


%By imposing certain constraints on the Lipschitz continuity of the score function, the assumption ensures a well-behaved and predictable behavior of the process.
In addition, Assumption \ref{ass:second_moment} introduces essential constraints on the moments of the target distribution. These constraints effectively prevent an excessive accumulation of probability mass in the tail region, thereby ensuring a more balanced and well-distributed target distribution. 
It should be noted that the first two assumptions are also introduced in diffusion analysis~\cite{chen2022sampling}. Besides, \ref{ass:lips_score} can be released to the smoothness of $p_0$ with more sophisticated techniques \citep{chen2023improved}. Assumption \ref{ass:convex_outside_ball} and \ref{ass:curve_outside_ball}  measure the tail behavior of the log density $f_*$. The convexity outside a ball follows the definition in \citep{ma2019sampling}.
%Assumption \ref{ass:convex_outside_ball} is nearly a  log-Sobolev distribution, but the log-Sobolev constant is usually small, e.g., Gaussian mixture. 
%Assumption \ref{ass:curve_outside_ball} is a general assumption that consider the quantify the degree of heavy tail distributions.
%To be more specific, Assumption \ref{ass:convex_outside_ball} covers the mixture model that can be simplified by $\textsc{rdMC}$, where the log-Sobolev constant can be reduced significantly.
%Assumption \ref{ass:curve_outside_ball} covers the heavy tail cases that Langevin-based algorithms cannot solve them numerically (such as $\exp(d)$-dependency).  


%These assumptions collectively provide a robust theoretical framework that guarantees the desirable properties of the underlying distributions involved in sampling problems. The careful consideration and incorporation of these assumptions contribute to the overall effectiveness and reliability of the proposed approach.
 %When it is dominated by the Gaussian tail, we can compute the log-Sobolev constants for all intermediate distributions.

% \subsection{Estimators of the Score and Choice of $T$}
\subsection{Convergence and Computation complexity of rdMC}
The log-Sobolev constant being close to zero or even absent altogether oftentimes represent the challenge in sampling problems.
A recent work on diffusion models \citep{chen2022sampling} hinted at the potential of the reverse diffusion process to circumvent this problem, given that the intermediary scores are estimated efficiently.
In particular, when Assumptions~\ref{ass:lips_score} and \ref{ass:second_moment} hold and when the estimator of the score is accurate enough, the iteration complexity of the score based reverse sampling algorithm is $\Theta(L^2 d\epsilon^{-2})$, which is independent of the log-Sobolev constant \xunp{why should we mention the gradient complexity of the inference process of diffusion models, our task is different}. 

In this section, we study whether the intermediary scores can be efficiently estimated via sampling from the initial distribution \(\hat{p}\) \xunp{what does this notation mean?} and the conditional one \(q_{T-t}\).
We also investigate how the numerical and statistical errors within each step will accumulate and affect the final accuracy.
For disposition purpose, we analyze Algorithm~\ref{alg:bpsa} with direct ULA sampling of $q_{T-t}(\cdot|\vx)$ described in Section~\ref{sec:score} and do not consider the smart importance sampling initialization (complexity of the importance sampling estimate is discussed in Section~\ref{sec:score})\xunp{you may not mention this issue over and over again}.

In our analysis, we first show in Theorem~\ref{thm:converge} below that when the error between the estimated distribution and the true \(\hat{p}\) \xunp{what does this notation mean?} and \(q_{T-t}\) adhere to certain conditions, by selecting an appropriate number of samples, our \textsc{rdMC} algorithm can approach the target distribution arbitrarily closely.



%For the issue of sampling, the primary computational burden arises from calculating $q_{T-t}$. It is worth mentioning that by selecting suitable values for \(T\) and \(\hat{p}\), we can tailor our approach to various problems. Theorem \ref{thm:converge} indicate that, with proper inner-loop accuracy and sample size, \textsc{rdMC} converge to the target distribution sufficiently close.

%For sampling task, we highlight that the 



%In practical scenarios, it is still unclear when  we can  estimated the score accurately. On the one hand, obtaining the oracle sampler for $q_t$ is often challenging, the concentration of the expectation may not be performed directly for implementable algorithms. Fortunately the density of $q_t$ is known, we can estimate the  mean with sampling methods.To guarantee the convergence of \textsc{rdMC} from a theoretical perspective, we consider the several possible implementable Step 5 in Alg~\ref{alg:bpsa}.


%we provide a detailed implementation of Step 5 in Alg~\ref{alg:bpsa} in the following.
%However, due to the difficulty of sampling beyond isoperimetry, the convergence rate we provided may not fully characterize the practical behavior. 
%\noindent\textbf{Importance sampling estimator.}



%With the following settings and the normal distribution is denoted as $C_0$
%\begin{small}
\iffalse
\begin{equation*}
    \begin{aligned}
        &\hat{\epsilon} = \exp\left(-32L\cdot 36^n \epsilon^{-8n}\right)\le \epsilon,\quad  \eta= C_1 (d+m_2^2)^{-1}\hat{\epsilon}^2,\quad a= \min\left\{2, -\frac{1}{2n}\log_{\epsilon}\left(\frac{-\ln \epsilon}{32L\cdot 36^n}\right)\right\}, \\
        &C_1 =2^{-9}\cdot 3^{-3}L^{-2},\quad C_2 =2^{-9}\cdot C_1^6 C_0^{-1},\quad C_3=2^{-20}C_0^{-2}C_1^{4},\quad \tilde{C}_{\mathrm{LSI}}= \frac{1}{6} \exp\left(-16\left(L+1\right)R^2\left(\frac{1}{6}\right)\right),\\
        & \tilde{q}_{T-k\eta}(\vx_0|\vx) \propto \exp\left(-f_*(\vx_0)- \frac{1}{2} \left\|\vx_0\right\|^2+\frac{e^{-(T-k\eta)}}{1-e^{-2(T-k\eta)}}\vx_0^\top \vx\right), 
    \end{aligned}
\end{equation*}
\fi
%\end{small}
%By performing the Unadjusted Langevin algorithm (ULA) in the inner loop to estimate $q_t$, and setting  parameters as following,

\begin{theorem}
%T = 2\ln\frac{\KL(p_*\Vert p_\infty)}{2\epsilon^2}
\label{thm:converge}
For any $\epsilon>0$, assume that $\KL(p_T\Vert \hat{p})<\epsilon$ for some $T>0$ and initialization $\hat p$ as suggested in Algorithm \ref{alg:bpsa}, $\eta = C_1(d+m_2^2)^{-1}\epsilon^2$.
    If the OU process induced by $p_*$ satisfies Assumption \ref{ass:lips_score}, \ref{ass:second_moment}, and $q_{T-k\eta}$ is log-Sobolev with constant $\mu_k$ ($k\eta\leq T$).
    We set
    \begin{equation}
\label{eq:setting}
    \begin{aligned}
     n_k = 64Td\mu_k^{-1}\eta^{-3}\epsilon^{-2}\delta^{-1},\quad \mathcal{E}_k = 2^{-13}\cdot T^{-4} d^{-2}\mu_k^2\eta^8\epsilon^{4}\delta^{4}
    \end{aligned}
\end{equation}
where $n_k$ is the number of samples to estimate the score, and $\mathcal{E}_k$ is the KL error tolerence for the inner loop. With probability at least
$1-\delta$, 
Algorithm \ref{alg:bpsa} converges in TV distance with $\tilde{O}(\epsilon)$ error.
\end{theorem}
%\textcolor{red}{Is $\hat{p}$ in Theorem 1 the same as $\hat{p}$ in Algorithm 1?}
%\textcolor{red}{Is $\mu$ the LSI constant of $P_T$?}


Theorem \ref{thm:converge} illustrates how the overall error of $\textsc{rdMC}$ depends on the accuracy of the inner loop score estimation step carried out by ULA. More importantly, for each inner loop, the complexity depend on the log-Sobolev constant of the $q_t$. 
% Lemma \ref{lem:log_sob} provide two potential estimates, that help us to understand the complexity of different $q_t$. 
% % For each step $k$,  $C_{\mathrm{LSI},k}$ is the log-Sobolev constant for the subproblem.
% %For each stage, Step 5 conducts a ULA whose log-Sobolev constant are shown in Table \ref{tab:log_sob}.

We then demonstrate that even if the target distribution $p_*$ does not satisfy the LSI, the conditional distribution \(q_{T-t}\) can still do.
We provide specific LSI constants for \(q_{T-t}\) with different $t$.
\begin{lemma}\label{lem:log_sob} For the forward OU process, we have the estimation of log-Sobolev constant as below
\begin{center}
\footnotesize
    \begin{tabular}{c|c|c}
    \toprule
     Assumptions &Interval  & LSI constant for $q_t$ \\
     \midrule
\ref{ass:lips_score}&$0\leq t\leq\frac{1}{2} \ln\left(1+\frac{1}{2L}\right)$ & $\frac{e^{-2t}}{2 \left(1-e^{-2t}\right)}$ \\\midrule
 \ref{ass:lips_score} and \ref{ass:curve_outside_ball}  &  $t\geq0$  & $\frac{e^{-2t}}{6(1-e^{-2t})}\cdot e^{-16\cdot 3L\cdot R^2\left(\frac{e^{-2t}}{6(1-e^{-2t})}\right)}$ \\
     \bottomrule
\end{tabular}.
\end{center}
The first estimation indicate that when $t$ is small, the quadratic induced term gives good log-Sobolev property. 
The tail property guarantees a uniform estimation but the bound is not always tight.
\end{lemma}



Lemma \ref{lem:log_sob} suggests that for $t\leq\frac{1}{2} \ln\left(1+\frac{1}{2L}\right)$, both $t$ and log-Sobolev constant are $O(1)$, which means the log-Sobolev properties for $q_t$ are well-behaved for small $t$. Moreover, we can also obtain that under weak tail assumption \ref{ass:curve_outside_ball}, %\textcolor{red}{(reference to which assumption?)}
all $q_t$ can be proven log-Sobolev, which is indicated by the quadratic term in $q_t$. 
That means even if $p_*$ does not satisfy LSI, we can still find a path towards $p_*$ to approximate it with any precision. \xunp{why should we put lemma 2 here? if it is only about [A4] we can throw it to Section 4.4}




%It is clear that the outer-loop iteration complexity is only $\tilde{O}(d\epsilon^{-2})$, which means the inner loop/score estimation is the main computation overhead for complex distributions. With importance sampling, the sample complexity is exponential in $d$. 
%With ULA inner loop, we may have the following convergence of Alg~\ref{alg:bpsa}, where the gradient complexity depend on the log-Sobolev constants of the sub-problems.
%Due to the space limitation, we defer the proof in Appendix~\ref{sec:main_proof_app}.


\subsection{Improving the Log-Sobolev constant dependence under Assumption~\ref{ass:convex_outside_ball}}

In what follows we study a case where $p_*$ admits a log-Sobolev constant, but scales exponentially with the radius of the region of nonconvexity. 
In \citep{ma2019sampling}, it is demonstrated that any distribution satisfying Assumptions~\ref{ass:lips_score} and \ref{ass:convex_outside_ball} has a log-Sobolev constant of $\frac{m}{2}\exp(-16LR^2)$, which scales exponentially with the radius $R$. 
In the Proposition~\ref{prop:log_sob_exp} below, we select values of \(T\) and \(\hat{p}\) to achieve the desired level of accuracy. Notably, if $T=O(\log R)$, the exponential dependency on $R$ can be reduced, which is very important for mixture models.
We find that the overall computation complexity of \textsc{rdMC} does not depend on the log-Sobolev constant. 
Instead, it depends only in a polynomial fashion on the radius of the region of nonconvexity.


\begin{proposition}
    \label{prop:log_sob_exp}
    Assume that the OU process induced by $p_*$ satisfies Assumption \ref{ass:lips_score}, \ref{ass:second_moment}, \ref{ass:convex_outside_ball}. 
    We estimate $p_T$ with $\hat{p}$ by the ULA inner loop, where the iteration complexity wrt log-Sobolev constant is $\Omega\left(m^{-1}\exp(16 LR^2 e^{-2T}-2T)\right)$.
    For any $\epsilon>0$ and $T\leq \frac{1}{2}\ln\left(1+\frac{1}{2L}\right)$, the Algorithm \ref{alg:bpsa} from $\hat{p}$ to target distribution convergence with a probability at least $1-\delta$ and total gradient complexity $\Omega\left(\mathrm{poly}(\epsilon,\delta)\right)$ independent of $R$.

    %For any $\epsilon>0$, by performing Algorithm \ref{alg:bpsa} with ULA inner loop, , we have  $\TVD\left(\tilde{p}_t, p_*\right) \le  \tilde{O}(\delta)$ with 
   
\end{proposition}


% Proposition \ref{prop:log_sob_exp} proves that our algorithm provide additional $\exp(-2T)$ shrinkage on $R^2$ to make the log-Sobolev well-behaved. In real practice, this property makes the algorithm easier to escape from different modes and reduce the barrier. Moreover, for some heavy-tailed distributions, our $q_t$ is always quadratic tail, which provides a feasible path to estimate them.


\noindent\textbf{Example: Gaussian Mixture Model.} We consider an example that $$p_*(x)\propto \exp\left(-\frac{1}{2}\Vert x\Vert^2\right)+
\exp\left(-\frac{1}{2}\Vert x-y\Vert^2\right),\quad y\gg1.$$
The log-Sobolev constant $\mu_0^{-1} \leq 1+\frac{1}{4}(e^{\Vert y\Vert^2}+1)$ \citep{schlichting2019poincare,menz2014poincare}. \citet{tosh2014lower} indicate that the iteration complexity lower bound of MCMC-based algorithm to sample from the Gaussian mixture scales exponentially with the squared distance $\|y\|^2$ between the two modes: $\Omega(\exp(\Vert y\Vert^2/8))$.  It is important to highlight that \textsc{rdMC} is a non-Markovian process, which convert the iteration complexity into sample complexity. With importance sampling score estimator, the $\tilde{O}(\epsilon^{-2})$ iteration complexity and $\tilde{O}(\epsilon^{-2})$ samples at each step, the TV distance converges with $\tilde{O}(\epsilon)$ error. The computation overhead of the whole process does not depend on $y$.  For the inner-loop score estimation we can choose $T = \frac{1}{2}\log \frac{3}{2}$ to make the log-Sobolev constant of $q_t$ to be $O(1)$. We also perform ULA to initialize $p_T$, which is close to $p_{\infty}$, the standard normal distribution. 
Specifically, the log-Sobolev constant of $p_T$ is $\mu_T^{-1}\leq 1+\frac{1}{4}(e^{\Vert e^{-T}y\Vert^2}+1)$, which improves the dependence on $\|y\|^2$ by a $e^{-2T} = \frac{2}{3}$ factor. 
Since this factor is on the exponent, the reduction is exponential.
See Appendix~\ref{sec:app_nota_ass} for the proof. 
\textcolor{red}{Make the symbols for the LSI constants consistent.}

Figure \ref{fig:gmm_mmd} provides an empirical demonstration for this example. We choose different radius $r$ to represent the change of $R$ in Assumption \ref{ass:convex_outside_ball}. We compare the convergence of Langevin Monte Carlo (LMC), Underdamped LMC (ULMC) and our algorithm in terms of gradient complexity. As \( r \) increases, we find that LMC fails to converge within a limited time. ULMC, with the introduction of velocity, can alleviate this situation. Notably, our algorithm can still ensure fast mixing even when \( r \) is very large. We choose $1,000$ particles in the experiments and choose $T = \log(5/4)$. We use $10$, $50$, or $100$ iterations to approximate $\hat{p}$ chosen by the corresponding problem. The inner loop contains $100$ particles initialize with importance sampling mean estimator. The inner iteration is chosen from $\{1,5\}$. The outer learning rate is chosen from $\{T/20,T/10,T/5\}$. When the algorithm converges, we further perform LMC until the limit of gradient complexity. See more empirical results in Appendix~\ref{}.
%\textcolor{red}{Throw more experimental settings into the appendix. Focus on the results.}


\subsection{Beyond Log-Sobolev inequality under Assumption~\ref{ass:curve_outside_ball}}

In the next Proposition~\ref{thm:main_con}, we study the case where the target distribution $p_*$ fails to satisfy LSI, but instead can have heavier tails as stipulated in Assumption~\ref{ass:curve_outside_ball}.
We find that in this case, an explicit computation complexity can still be obtained for \textsc{rdMC} to converge to any desired accuracy.
Although admittedly its dependence on $1/\epsilon$ is exponential.
\begin{proposition}
    \label{thm:main_con}
    Assume that the target distribution $p_*$ satisfies Assumption \ref{ass:lips_score}, \ref{ass:second_moment}, and \ref{ass:curve_outside_ball}. 
    We take $p_\infty$ to be $\hat{p}$.
    For any $\epsilon>0$, by performing Algorithm \ref{alg:bpsa} with ULA inner loop and hyper-parameters in Theorem \ref{thm:converge}, with a probability at least $1-\delta$, we have  $\TVD\left(\tilde{p}_t, p_*\right) \le  \tilde{O}(\epsilon)$ with 
    $\Omega\left(d^{18}\epsilon^{-16n-83}\delta^{-6}\exp\left(\epsilon^{-16n}\right)\right)$
 gradient complexity.
\end{proposition}
%It should be notice that when \ref{ass:curve_outside_ball_v2} holds, the complexity of the sampling task can be just polynomial, since negative curvature of the log-density is dominated by a polynomial function. 
%\textcolor{red}{Do you wanna specify the choice of $n$ here?}


%(see e.g., Theorem 3.16 of Martin Wainwright's book ``High-dimensional statistics'').

%This Lipschitzness seems to be a mild assumption on $f_*(\vx_0)$.



%\section{Examples}



\noindent\textbf{Example: Heavy-tailed distribution beyond isoperimetry.}
Instead of requiring the isoperimetry in most previous analysis~\cite{vempala2019rapid,ma2021there}, we introduce~\ref{ass:curve_outside_ball} to analyze \textsc{rdMC} convergence in a more general class of target distributions.
Intuitively, it allows the negative log density, i.e., $f_*$, to have a slow growth rate beyond a bounded region, which also implies the tail of $p_*$ can be heavier.

On the other hand, if $p_*$ satisfies LSI, then according to Proposition 5.4.1 in~\cite{bakry2014analysis} there exists some $\sigma>0$ such that
$
    \int \exp\left(-f_*(\vx)+\frac{\sigma^2}{2}\left\|\vx\right\|^2\right)\der \vx <\infty.$
Thus, it is equivalent to a quadratic growth of $f_*$ outside a ball, which is more stringent than~\ref{ass:curve_outside_ball}.
Besides, a sufficient condition to make $p_*$ satisfy Poincar\'e inequality is the distant dissipativity condition~\citep{bakry2008simple}:
$
    \left<\vx, \grad f_*(\vx)\right> \ge a\left\|\vx\right\|\quad \text{holds when}\ \left\|\vx\right\|\ge R
$
for some $a, R>0$. 
The previous assumption fails when the growth of $f_*$ is sub-linear.

\textbf{More discussion with weak PI}


We consider for example a $1$-d distribution with density:
 $p_*(x)\propto \exp\left(-\left(x^2+1\right)^{1/4}\right).$
Due to its tail being heavier than Gaussian distributions, $p_*$ violates the the previous conditions, breaking both log-Sobolev and Poincar\'e inequalities. 
However, we know $p_*$ has a bounded second moment, and its negative density function satisfies $
\left|\grad^2 f_*(x)\right|=\left|\frac{1}{4}\cdot (2-x^2)\cdot \left(x^2+1\right)^{-7/4}\right|\le \frac{1}{2}.$
It can be further proven that $p_*$ satisfies Assumption~\ref{ass:curve_outside_ball}, with detailed proof deferred to Appendix~\ref{sec:app_nota_ass}.







\begin{figure}
    \centering
    \begin{tabular}{ccc}
          \includegraphics[width=4.2cm]{figs/R_0.5_.pdf} & \includegraphics[width=4.2cm]{figs/R_1_.pdf} & 
          \includegraphics[width=4.2cm]{figs/R_2_.pdf} \\
          \includegraphics[width=4.2cm]{figs/r05_gmm.pdf} & \includegraphics[width=4.2cm]{figs/r1_gmm.pdf} & 
          \includegraphics[width=4.2cm]{figs/r2_gmm.pdf} \\
          $r=0.5$& $r=1.0$&$r=2.0$
    \end{tabular}
    \caption{Maximum Mean Discrepancy (MMD) convergence of LMC, ULMC, \textsc{rdMC}. The first row shows different target distributions, with increasing \( r \) leading to a reduced log-Sobolev constant and greater barriers between modes. The second row highlights the algorithmic convergence, revealing rdMC's pronounced advantage convergence compared to ULMC/LMC, especially for large \( r \) values.%\textcolor{red}{Add a few sentences to explain the figure. Walk the readers through the figure: what do the top and bottom panels show etc.} 
    }
    \label{fig:gmm_mmd}
\end{figure}
%the log-Sobolev constant for $q_t$ is $\frac{e^{-2(T-t)}}{2(1-e^{-2(T-t)})}$.



%Let $t=\Vert y\Vert^2/2\sigma^2$, $\mu_t^{-1} = O(1)$.

%We have $-\log p_*(x) = -\log \left(\exp\left(-\frac{1}{2}\Vert x\Vert^2\right)+\exp\left(-\frac{1}{2}\Vert x-y\Vert^2\right)\right)$

%then $$\frac{d^2}{dx^2}(-\log p_*(x)) = 1-\frac{y^2 e^{\frac{y (y + 2 x)}{2 }}}{(e^{\frac{y^2}{2 }} + e^{{y x}})^2}$$



\iffalse
$$
q_{T-t}(x_0|x) \propto \exp\left(\log \left(\exp\left(-\frac{1}{2\sigma^2}\Vert x_0\Vert^2\right)+
\exp\left(-\frac{1}{2\sigma^2}\Vert x_0-y\Vert^2\right)\right)
- \frac{\Vert x-e^{-(T-t)}x_0\Vert^2}{2(1-e^{-2(T-t)})}
\right)
$$
The corresponding log-Sobolev constant is 
$$
\mu^{-1}_T \lesssim
$$


$$
p_{T-t} = \left(\exp\left(-\frac{1}{2(1-(1-\sigma^2)e^{-2(T-t)})}\Vert   x\Vert^2\right)+
\exp\left(-\frac{1}{2(1-(1-\sigma^2)e^{-2(T-t)})}\Vert  x-ye^{-(T-t)}\Vert^2\right)\right) 
$$
The corresponding log-Sobolev constant is 
$$
\nu_T^{-1}\lesssim \exp\left(
\frac{e^{-2T}\Vert y\Vert^2}{1-(1-\sigma^2)e^{-2T}}
\right)\leq 
\exp\left(
\frac{e^{-2T}\Vert y\Vert^2}{1-e^{-2T}}
\right)
$$
\fi




==> 0_contents/backup.tex <==
\section{Our Algorithms}
This draft provides a novel sampling method inspired by the denoising diffusion model. 
Similar to diffusion models, consider Ornstein-Uhlenbeck(OU) process as the forward process, i.e.,
\begin{equation}
    \label{eq:ou_sde}
    \der \rvx_t = -\rvx_t \der t + \sqrt{2}\der B_t,\quad \rvx_0\sim p_* \propto e^{-f_*},
\end{equation}
where $(B_t)_{t\ge 0}$ is Brownian motion in $\R^d$.
Similar to Eq.(4) in~\cite{chen2022sampling}, if we fix the terminal time $T>0$ and set
\begin{equation*}
    \hat{\rvx}_t = \rvx_{T-t}, \quad \mathrm{for}\ t\in[0, T],
\end{equation*}
reverse the process, or we say the backward path can be presented as
\begin{equation*}
    \der \hat{\rvx}_t = \left(\hat{\rvx}_t + 2\grad\ln p_{T-t}(\hat{\rvx}_t)\right)\der t + \sqrt{2}\der B_t,
\end{equation*}
where $p_t$ denotes the underlying distribution of the particle $\rvx_t$, and we require $\hat{\rvx}_0 \sim p_T$.
By setting
\begin{equation}
    \label{def:g}
    g(\vx, t) = - \vx - 2\grad \ln p_{T-t}(\vx),
\end{equation}
the particles' update with Euler's method is 
\begin{equation*}
    \hat{\rvx}_{k+1} = \hat{\rvx}_k -\eta_k g\left(\hat{\rvx}_k, \sum_{i=1}^{k-1}\eta_i\right) + \sqrt{2\eta_k}\mathcal{N}(0, \mI), 
\end{equation*}
when the step size is a constant $\eta$, we have
\begin{equation}
    \label{ite:paticle_2}
    \hat{\rvx}_{k+1} = \hat{\rvx}_k -\eta g\left(\hat{\rvx}_k, (k-1)\eta\right) + \sqrt{2\eta}\mathcal{N}(0, \mI).
\end{equation}
Thus, we start to approximate the term $g(\cdot)$.
\paragraph{Approximate the Drift Term of the Backward Path}
When the OU process, i.e., Eq.~\ref{eq:ou_sde}, is selected as our forward path, the transition kernel of $(\rvx_t)_{t\ge 0}$ has a closed form, i.e.,
\begin{equation*}
    p(\vx, t | \vx^\prime, t^\prime) = \left(2\pi \left(1-e^{-2(t - t^\prime)}\right)\right)^{-d/2}
     \cdot \exp \left[\frac{-\left\|\vx -e^{-(t -t^\prime)}\vx^\prime \right\|^2}{2\left(1-e^{-2(t -t^\prime)}\right)}\right], \quad \forall\ 0\le t^\prime\le t\le T.
\end{equation*}
In this condition, we set $t^\prime = t+\Delta t$, and have
\begin{equation*}
    \begin{aligned}
    p_{T-t}(\vx) = &\int_{\R^d} p_{T-t^\prime}(\vx^\prime) \cdot p_{T-t|T-t^\prime}(\vx|\vx^\prime)\der \vx^\prime\\
    = & \int_{\R^d} p_{T-t^\prime}(\vx^\prime)\cdot \left(2\pi \left(1-e^{-2\Delta t}\right)\right)^{-d/2} \cdot \exp\left(-\frac{\left\|\vx - e^{-\Delta t}\vx^\prime\right\|^2}{2\left(1-e^{-2\Delta t}\right)}\right)\der \vx^\prime
    \end{aligned}
\end{equation*}
Besides, we have
\begin{equation*}
    \grad_{\vx} \ln p_t(\vx) = \frac{\grad_{\vx} p_t(\vx)}{p_t(\vx)},
\end{equation*}
and plug the formulation of $p_t$ into this equation. We obtain
\begin{equation}
    \label{equ:grad_ln_pt}
    \begin{aligned}
        \grad_{\vx} \ln p_{T-t}(\vx) = &\frac{\grad \int_{\R^d} p_{T-t^\prime}(\vx^\prime)\cdot \left(2\pi \left(1-e^{-2\Delta t}\right)\right)^{-d/2} \cdot \exp\left(-\frac{\left\|\vx - e^{-\Delta t}\vx^\prime\right\|^2}{2\left(1-e^{-2\Delta t}\right)}\right)\der \vx^\prime}{\int_{\R^d} p_{T-t^\prime}(\vx^\prime)\cdot \left(2\pi \left(1-e^{-2\Delta t}\right)\right)^{-d/2} \cdot \exp\left(-\frac{\left\|\vx - e^{-\Delta t}\vx^\prime\right\|^2}{2\left(1-e^{-2\Delta t}\right)}\right)\der \vx^\prime}\\
        = &\frac{\int_{\R^d} p_{T-t^\prime}(\vx^\prime) \cdot \exp\left(-\frac{\left\|\vx - e^{-\Delta t}\vx^\prime\right\|^2}{2\left(1-e^{-2\Delta t}\right)}\right) \cdot \left(-\frac{\vx - e^{-\Delta t }\vx^\prime}{1-e^{-2\Delta t}}\right)\der \vx^\prime}{\int_{\R^d} p_{T-t^\prime}(\vx^\prime)\cdot \exp\left(-\frac{\left\|\vx - e^{-\Delta t}\vx^\prime\right\|^2}{2\left(1-e^{-2\Delta t}\right)}\right)\der \vx^\prime}\\
        = & \mathbb{E}_{\rvx^\prime \sim \hat{p}_t}\left[-\frac{\vx - e^{-\Delta t }\rvx^\prime}{1-e^{-2\Delta t}}\right]
    \end{aligned}
\end{equation}
where the density function $\hat{p}_t$ is defined as
\begin{equation*}
    \hat{p}_t(\vx^\prime) = \frac{p_{T-t^\prime}(\vx^\prime) \cdot \exp\left(-\frac{\left\|\vx - e^{-\Delta t}\vx^\prime\right\|^2}{2\left(1-e^{-2\Delta t}\right)}\right)}{\int_{\R^d} p_{T-t^\prime}(\vx^\prime)\cdot \exp\left(-\frac{\left\|\vx - e^{-\Delta t}\vx^\prime\right\|^2}{2\left(1-e^{-2\Delta t}\right)}\right)\der \vx^\prime}.
\end{equation*}
Similar to~\cite{chen2022sampling}, we suppose $\log p_t\coloneqq -f_t$ and assume $\grad f_t$ is $L$-Lipschitz for convenience (this assumption may be removed in the latter proof).
In this condition, we may rewrite $\hat{p}_t(\vw)$ as 
\begin{equation*}
    \hat{p}_t(\vx^\prime) = \frac{ \exp\left(-f_{T-t^\prime}(\vx^\prime)-\frac{\left\|\vx - e^{-\Delta t}\vx^\prime\right\|^2}{2\left(1-e^{-2\Delta t}\right)}\right)}{\int_{\R^d} \exp\left(- f_{T-t^\prime}(\vx^\prime)-\frac{\left\|\vx - e^{-\Delta t}\vx^\prime\right\|^2}{2\left(1-e^{-2\Delta t}\right)}\right)\der \vx^\prime}\propto \exp\left(-f_{T-t^\prime}(\vx^\prime)-\frac{\left\|\vx - e^{-\Delta t}\vx^\prime\right\|^2}{2\left(1-e^{-2\Delta t}\right)}\right).
\end{equation*}
According to Eq.~\ref{ite:paticle_2}, Eq.~\ref{def:g} and Eq.~\ref{equ:grad_ln_pt}, if we can sample from $\hat{p}_t$, then we can obtain approximation of $g(\cdot, (k-1)\eta)$ by estimating $\mathbb{E}_{\rvx^\prime \sim \hat{p}_t}\left[- (\vx - e^{-\Delta t }\rvx^\prime)/({1-e^{-2\Delta t}})\right]$.
In the following, I will show how to sample from $\hat{p}_t$ which is equivalent to the implementation of the Restricted Gaussian Oracle(RGO).

\paragraph{Sampling from auxiliary distribution $\hat{p}_t$}
In this part, we utilize similar techniques as~\cite{liang2022proximal} which aims to solve the following problem, i.e.,
\begin{definition}(RGO problem)
Given a point $\vy\in\R^d$ and step size $\eta>0$, a restricted Gaussian oracle (RGO) for convex $f\colon \R^d \rightarrow \R$ is a sampling oracle that returns a sample from a distribution proportional to 
\begin{equation}
    \label{def:rgo_target}
    \exp\left(-f(\cdot)-\frac{1}{2\eta}\left\|\cdot - \vy\right\|^2\right).
\end{equation}
\end{definition}
Therefore, we should reformulate $\hat{p}_t$ into Eq.~\ref{def:rgo_target} by choosing
\begin{equation*}
    \Delta t\le \frac{1}{2}\cdot \ln \frac{1+2L}{2L},
\end{equation*}
then we have
\begin{equation*}
    \hat{f}_{T-t^\prime}(\vx^\prime) = f_{T-t^\prime}(\vx^\prime) + \frac{\left\|\vx-e^{-\Delta t}\vx^\prime\right\|^2}{4(1-e^{-2\Delta t})},
\end{equation*}
which has $\grad^2 f^\prime_{T-t^\prime}(\vx^\prime)\succeq 0$, and 
\begin{equation*}
    \hat{p}_t(\vx^\prime) \propto \exp\left(-\hat{f}_{T-t^\prime}(\vx^\prime) - \frac{\left\|\vx - e^{-\Delta t}\vx^\prime\right\|^2}{2\left(1-e^{-4\Delta t}\right)}\right)
\end{equation*}
where $f^\prime_{T-t}$ is convex.
This formulation matches Eq.~\ref{def:rgo_target}. 
We should note that in this setting $\log \hat{p}_t$ is a well-conditioned density function, whose condition number will be close to $\kappa = 2$.

\textcolor{blue}{Currently, the problem may be the difficulties in obtaining the function value and gradient of $\hat{f}_{T-t}$, once these values can be estimated efficiently, the whole algorithm is completed. 
Noted that, 
While this problem may be solved by this \href{https://dsp.stackexchange.com/questions/76320/fast-computation-of-a-convolution-integral-with-gaussian-kernel}{link} }


%According to Lemma~\ref{lem:stable_prod}, we know $(\rvx_0^{(1)},\ldots, \rvx_0^{(N_k)})\sim \left(q_{T-k\eta}^\prime\right)^{\otimes N_k}$ where  $\left(q_{T-k\eta}^\prime\right)^{\otimes N_k}$ shares the same LSI contant with $q_{T-k\eta}^\prime$.
%We define the function 
%which establishes due to the triangle inequality of the norm.
%Therefore, with Lemma~\ref{lem:lsi_concentration} and the $0.5\Sigma_{\min}$-LSI for $q_{T-k\eta}^\prime$, we have
%\begin{equation*}
%    \begin{aligned}
%        &\mathrm{Pr}\left\{\left\|\sum_{i=1}^{N_k}\rvx_0^{(i)} \right\| \ge \mathbb{E}\left[\left\| \sum_{i=1}^{N_k}\rvx_0^{(i)}\right\|\right]+ \frac{1-e^{-(T-k\eta)}}{2e^{-(T-k\eta)}} \cdot N_k \Delta\right\} \le \exp\left(-\frac{\left(1-e^{-(T-k\eta)}\right)^2 N_k^2 \Delta^2 \Sigma_{\min}}{16 \cdot e^{-2(T-k\eta)}}\right)\\
%        \Rightarrow & \mathrm{Pr}\left\{\left\|\frac{1}{N_k}\sum_{i=1}^{N_k}\rvv_i - \frac{1}{N_k}\mathbb{E}\left[\sum_{i=1}^{N_k}\rvv_i\right]\right\| \ge \Delta\right\} \le \exp\left(-\frac{\left(1-e^{-(T-k\eta)}\right)^2 N_k^2 \Delta^2 \Sigma_{\min}}{16 \cdot e^{-2(T-k\eta)}}\right)\\
%        & \qquad =  \exp\left(-\frac{1}{32}\cdot \frac{1-e^{-(T-k\eta)}}{2\sigma^2}\cdot N_k^2 \Delta^2\right) \le \exp\left(-\frac{1}{32}\cdot \left(1-e^{-\eta}\right)\cdot \frac{LC^4}{32\epsilon^4}\cdot N_k^2 \Delta^2\right)
 %   \end{aligned}
%\end{equation*}
%By choosing $\Delta = 4\epsilon^3/(\sqrt{L}C^2)$, we have
%\begin{equation*}
%    \mathrm{Pr}\left[\left\|\rvv_k(\vx) - \int q_{T-k\eta}^\prime(\vx_0)(-2)\cdot \frac{\vx - e^{T-k\eta}\vx_0}{1-e^{-2(T-k\eta)}}\right\|^2 \le \frac{16\epsilon^6}{LC^4}\right] \ge 1-\exp \left(- \frac{1-e^{-\eta}}{2} \cdot N_k^2 \epsilon^2\right).
%\end{equation*}
%That means choosing 
%\begin{equation}
%    \label{ineq:choice_of_Nk}
%    N_k\ge \sqrt{\lfloor T/\eta \rfloor} \sqrt{\frac{2}{1-e^{-\eta}}}\cdot %\epsilon^{-1.5} 
%\end{equation}


Then, we solve the proximal bundle subproblem with Alg~\ref{alg:spbs}.
\begin{algorithm}[!hbpt]
    \caption{Solving the Proximal Bundle Subproblem}
    \label{alg:spbs}
    \begin{algorithmic}[1]
            \STATE {\bfseries Input:} Let $y,\hat{\eta}>0$ and $\delta>0$ be given, and set $\tilde{\vx}_0 = e^{(T-t)}\vx$, $C_1=\{\tilde{\vx}_0\}$ and $j=1$;
            \STATE Update $l_j = \max\left\{\hat{l}_{T-t}(\tilde{\vx})+ \left<\grad \hat{l}_{T-t}(\tilde{\vx}),\cdot - \tilde{\vx}\right>, \tilde{\vx}\in C_j\right\}$;
            \STATE Compute
            \begin{equation}
                \begin{aligned}
                \vx_j = &\argmin_{\vu\in\R^d}\left\{g_j^{\hat{\eta}}\coloneqq l_j(\vu) + \frac{\mu}{2}\cdot \left\|\vu - e^{(T-t)}\vx\right\|^2+\frac{1}{2\hat{\eta}}\|\vu - e^{(T-t)}\vx\|^2\right\}\\
                \tilde{\vx}_j\in & \argmin \left\{g_{T-t}(\vu), \vu\in\{\vx_j, \tilde{\vx}_j\}\right\};
                \end{aligned}
            \end{equation}
            \STATE If $\hat{g}_{T-t}(\tilde{\vx}_j) - g^{\hat{\eta}}_j(\vx_j)\le \delta$ then \textbf{stop}; else go to step 5;
            \STATE Choose $C_{j+1}$ such that
            \begin{equation*}
                A_j\cup \{\vx_j\} \subseteq C_{j+1}\subseteq C_j\cup \{\vx_j\}
            \end{equation*}
            where $A_j = \left\{l_j(\vx_j) = \hat{l}_{T-t}(\tilde{x})+\left<\grad \hat{l}_{T-t}(\tilde{\vx}), \vx_j -\tilde{\vx}\right>, \tilde{\vx}\in C_j\right\}$;
            \STATE Set $j\leftarrow j+1$ and go to step 2.
    \end{algorithmic}
\end{algorithm}
When this algorithm return, we utilize the variable obtained at the last step to construct the following function
\begin{equation*}
    h_1 \coloneqq \frac{1}{2\hat{\eta}_\mu}\left\|\cdot - \vx_j\right\|^2+\hat{g}_{T-t}(\tilde{\vx}_j)-\delta,
\end{equation*}
and solve the RGO problem with the following algorithm
\begin{algorithm}[!hbpt]
    \caption{Implementable RGO without optimization oracle}
    \label{alg:rgo_non_orc}
    \begin{algorithmic}[1]
            \STATE Compute $\vx_j$ and $\tilde{\vx}_j$ with Alg~\ref{alg:spbs};
            \STATE Generate $\rvx\sim \exp(-h_1(\vx))$;
            \STATE Generate $\rvu\sim \mathcal{U}[0,1]$;
            \STATE If 
            \begin{equation*}
                \rvu\le \frac{\exp(-g_{T-t}(\rvx))}{\exp(-h_1(\rvx))},
            \end{equation*}
            then accept $\tilde{\rvx}=\rvx$; else reject $\rvx$  and go to step.2.
    \end{algorithmic}
\end{algorithm}




\paragraph{Reformulate the auxiliary sampling task}
In this part, we utilize similar techniques as~\cite{liang2022proximal} which aims to solve the following problem, i.e.,
\begin{definition}(RGO problem)
Given a point $\vy\in\R^d$ and step size $\eta>0$, a restricted Gaussian oracle (RGO) for convex $f\colon \R^d \rightarrow \R$ is a sampling oracle that returns a sample from a distribution proportional to 
\begin{equation}
    \label{def:rgo_target}
    \exp\left(-g(\cdot)-\frac{1}{2\eta}\left\|\cdot - \vy\right\|^2\right).
\end{equation}
\end{definition}
Therefore, we expect to reformulate $q_{T-t}$ into Eq.~\ref{def:rgo_target}.


\begin{theorem}
For Term 1 of Eq.~\ref{ineq:main}, assume that $C_\sigma=\KL\left(p_0\| p_\infty\right)$. When we choose the $T=2\ln(C_\sigma/2\epsilon^2)$, we have
\begin{equation*}
    \begin{aligned}
        \sqrt{\frac{1}{2}\KL\left(p_T\|p_\infty\right)}<\epsilon .
    \end{aligned}
\end{equation*}
The analysis is provided in Section~\ref{sec:analysis_forward}. 
\end{theorem}

==> 0_contents/other_comments.tex <==

\subsection{How small is the denominator?}
Assume that we have aligned the functions so that $\min_{x_0} f_*(x_0) \approx 0$.
Also assume that function $f_*$ is $L$-Lipschitz smooth.
Then $\exp(-f_*(x_0)) \geq \exp\left( -\frac{L}{2} \left\| x_0-x_0^* \right\|^2 \right)$.
Therefore, 
\begin{align*}
\mathbb{E}_{\rvx_0 \sim \rho_{T-t}(\cdot|\vx)}\left[ \exp(-f_*(\vx_0))\right]
&\geq \frac{ \int \exp\left( -\frac{\left\|\vx - e^{-(T-t)}\vx_0\right\|^2}{2\left(1-e^{-2(T-t)}\right)} -\frac{L}{2} \left\| x_0-x_0^* \right\|^2 \right) \rd x_0 }{ \int \exp\left( -\frac{\left\|\vx - e^{-(T-t)}\vx_0\right\|^2}{2\left(1-e^{-2(T-t)}\right)} \right) \rd x_0 } \\
&= \left( \frac{\alpha}{\alpha+L} \right)^{d/2} \exp\left( - \frac{1}{2} \frac{\alpha L}{\alpha+L} \left\| e^{T-t} x - x_0^* \right\|^2 \right).
\end{align*}
where $\alpha = \frac{e^{-2(T-t)}}{1-e^{-2(T-t)}}$, and the last equality is obtain via completing the squares:
\begin{align*}
\frac{\left\|\vx - e^{-(T-t)}\vx_0\right\|^2}{\left(1-e^{-2(T-t)}\right)} + L \left\| x_0-x_0^* \right\|^2
= (\alpha+L) \left\| x_0 - \frac{\alpha e^{T-t}x + L x_0^*}{\alpha+L} \right\|^2
+ \frac{\alpha L}{\alpha+L} \left\| e^{T-t} x - x_0^* \right\|^2.
\end{align*}
We note that when $T-t$ is large, $\alpha$ is exponentially small.
Hence $\frac{\alpha}{\alpha + L} \approx \frac{\alpha}{L} \approx \frac{e^{-2(T-t)}}{L}$ and $\frac{\alpha L}{\alpha + L} \approx e^{-2(T-t)}$.
Therefore,
\[
\mathbb{E}_{\rvx_0 \sim \rho_{T-t}(\cdot|\vx)}\left[ \exp(-f_*(\vx_0))\right]
\gtrsim L^{-d/2} \cdot e^{-d(T-t)} \cdot e^{ -\frac{1}{2} \left\| x-e^{-(T-t)}x_0^* \right\|^2 }.
\]




\section{Can we use the varitional lower bound?}
We know that estimating 
\begin{align*}
\mathbb{E}_{\rvx_0 \sim \rho_{T-t}(\cdot|\vx)}\left[-\frac{\vx - e^{-(T-t)}\rvx_0}{\left(1-e^{-2(T-t)}\right)} \cdot \exp(-f_*(\vx_0))\right]
\Bigg/
\mathbb{E}_{\rvx_0 \sim \rho_{T-t}(\cdot|\vx)}\left[ \exp(-f_*(\vx_0))\right]
\end{align*}
is difficult.
What if we instead use a variational lower bound approach: $\mathbb{E}_{x}[g(x)] \geq \exp\left( \mathbb{E}_{x}[\log g(x)] \right)$ and estimate the lower bound instead?

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

